Low Degree Testing over the Reals

We study the problem of testing whether a function $f: \mathbb{R}^n \to \mathbb{R}$ is a polynomial of degree at most $d$ in the \emph{distribution-free} testing model. Here, the distance between functions is measured with respect to an unknown distribution $\mathcal{D}$ over $\mathbb{R}^n$ from which we can draw samples. In contrast to previous work, we do not assume that $\mathcal{D}$ has finite support. We design a tester that given query access to $f$, and sample access to $\mathcal{D}$, makes $(d/\varepsilon)^{O(1)}$ many queries to $f$, accepts with probability $1$ if $f$ is a polynomial of degree $d$, and rejects with probability at least $2/3$ if every degree-$d$ polynomial $P$ disagrees with $f$ on a set of mass at least $\varepsilon$ with respect to $\mathcal{D}$. Our result also holds under mild assumptions when we receive only a polynomial number of bits of precision for each query to $f$, or when $f$ can only be queried on rational points representable using a logarithmic number of bits. Along the way, we prove a new stability theorem for multivariate polynomials that may be of independent interest.

==> old_characterizations_of_polys.tex <==

\begin{thm}\label{thm:Usefulchar}
     Let $f:\mathbb{R}^n\rightarrow \mathbb{R}$ be an analytic function and $d$ be a non-negative integer. Then, $f$ is a degree-$d$ polynomial if and only if for every $\bm a, \bm b \in \mathbb{R}^n$ and  $t_1,\ldots, t_d \in \mathbb{R} \setminus \{0\}$ and every $e \in \mathbb{R}$, the following holds:
    \[\sum_{S\subseteq\{t_1,\hdots,t_d\}} (-1)^{|S|}f\Big(\bm{a} +\big(e+t_S\big)\bm{b} \Big)=\sum_{S\subseteq\{t_1,\hdots,t_d\}} (-1)^{|S|}f\Big(\bm{a} +t_S\bm{b} \Big),\] where $t_S = \sum_{t_j \in S}t_j$. 
\end{thm}



The proof will follow by the next two  lemmas; the first of which characterizes degree-$d$ multivariate polynomials by their restrictions to all such lines. % (oblivious to analyticity of $f$): 

\begin{lem}\label{lem:localmulti} 
    An analytic function $f:\mathbb{R}^n\rightarrow\mathbb{R}$ is a degree-$d$ polynomial if and only if for every $\bm{a},\bm{b}\in\mathbb{R}^n$, $f_{\bm{a},\bm{b}}$ is a degree-$d$ (univariate) polynomial.
\end{lem}
The second lemma characterizes degree-$d$ univariate polynomials.

\begin{lem}[Local characterization of univariate polynomials]\label{lem:localuni}
    An analytic function $g:\mathbb{R}\rightarrow\mathbb{R}$ is a degree-$d$ polynomial if and only if for every $t_1,\hdots,t_d\in\mathbb{R}\setminus\{0\},\forall e\in\mathbb{R}:$
    $$\sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}g\Big(e +t_S \Big)=\sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}g\Big(t_S \Big),$$
    where $t_S = \sum_{t_j \in S}t_j$.
\end{lem}
Assuming these lemmas, we establish the characterization.

\begin{proof}[Proof of \autoref{thm:Usefulchar}]
    Let $f:\mathbb{R}^n\rightarrow\mathbb{R}$ be an analytic function. By \autoref{lem:localmulti}, $f$ is a degree-$d$ polynomial if and only if for every $\bm a, \bm b \in \mathbb{R}^n$ the projection of $f$ onto the line $L_{\bm a,\bm b}$, $f_{\bm a, \bm b}(x) = f(\bm a + x \bm b)$ is itself a degree-$d$ (univariate) polynomial. By \autoref{lem:localuni}, this is equivalent to the following: for every  $t_1,\ldots, t_d \in \mathbb{R} \setminus \{0\}$, and every $e \in \mathbb{R}$, 
    \begin{align*}
        \sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}f_{\bm{a},\bm{b}}\Big(e +t_S \Big)& =\sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}f_{\bm{a},\bm{b}}\Big(t_S \Big) \\ &=\sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}f\Big(\bm{a} +\big(e+t_S\big)\bm{b} \Big) \\
        &=\sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}f\Big(\bm{a} +t_S\bm{b} \Big). 
        \qedhere
    \end{align*}
\end{proof}

In the remainder of this section we prove \autoref{lem:localmulti} and  \autoref{lem:localuni}.

\begin{proof}[Proof of \autoref{lem:localmulti}]
    $(\Rightarrow)$ 
    Fix $\bm{a},\bm{b} \in\mathbb{R}^n$, and note that $f_{\bm{a},\bm{b}}(x) = f(\bm a + x \bm b)$ is a univariate polynomial. 
    For any monomial of $f$ with degree $k$, the degree of the polynomial obtained from the monomial by replacing $x$ with $\bm{a}+x\bm{b}$, is at most $k$. Thus, the degree of $f_{\bm{a},\bm{b}}$ is at most $d$.
    \\
    $(\Leftarrow)$ 
    We will prove that $f$ is a degree-$d$ polynomial, by induction on $n$.
    For the base case, when $n=1$,  
    let $a \in \mathbb{R}$ be arbitrary, and let $b \neq 0$.
    Then, $f(x)=f_{a,b}((x-a)/b)$, which is a degree-$d$ polynomial from the premise.
    \\
    Suppose that the inductive hypothesis holds for $n-1$. 
    For $e \in \mathbb{R}$, let $f_{e}:\mathbb{R}^{n-1}\rightarrow\mathbb{R}$ be the $(n-1)$-variate function defined as $f_{e}(a_1,\ldots,a_{n-1}) \triangleq f(a_1,\ldots,a_{n-1},e)$. We will argue that $f_e$ is a degree-$d$ polynomial. Fix any $\bm{a}, \bm{b} \in \mathbb{R}^{n-1}$, and let  $\bm{a'}, \bm{b'} \in \mathbb{R}^{n}$ extend $\bm{a}$ and $\bm{b}$ respectively by setting $\bm{a'}_n \triangleq e$ and $\bm{b'}_n \triangleq 0$ respectively. Then $f_{\bm{a'},\bm{b'}}$ is a degree-$d$ univariate polynomial by assumption. Observe that
    \[
    f_{\bm{a'},\bm{b'}}(x) = 
    f(a_1+x_1b_1,\ldots, a_{n-1}+x_{n-1}b_{n-1}, e) = f_e(a_1+x_1b_1,\ldots, a_{n-1}+x_{n-1}b_{n-1}) = f_{e,\bm{a},\bm{b}}(x), \]
    which proves that for every $\bm{a}, \bm{b} \in \mathbb{R}^{n-1}$ $f_{e,\bm{a},\bm{b}}$ is a degree-$d$ univariate polynomial. By the inductive hypothesis, $f_e$ is a degree-$d$ polynomial.
    \\
    Next, we claim that $f$ is a polynomial of degree at most $2d$.
    \begin{clm}
        For $e \in \{0,\ldots,d\}$ define $\delta_{e}: \mathbb{R}\to \mathbb{R}$ to be the unique, degree-$d$ polynomial such that $\delta_{e}(e)=1$ and $\delta_{e}(e')=0$, for $e'\in\{0,\ldots,d\}\setminus\{e\}$. Then $f$ can be expressed as
        \[f(x)=\sum_{e=0}^{d}\delta_{e}(x_n)\cdot\underbrace{f_{e}(x_1,x_2,\ldots,x_{n-1})}_{degree=d}.\]
        In particular, $f$ is a degree-$2d$ polynomial.
    \end{clm}
    \begin{proof}
        Fix any $c_1,\ldots, c_{n-1} \in\mathbb{R}$.
        We first show, for every $t\in\mathbb{R}$,
        $$f(c_1,\ldots,c_{n-1},t)=\sum_{e=0}^{d}\delta_{e}(t)\cdot \underbrace{f_{e}(c_1,\ldots,c_{n-1})}_{deg_{t}(f_e)=0}.$$
        Observe that that both sides of the equation are degree-$d$ univariate polynomials in the variable $t$; indeed, $f(c_1,\ldots, c_{n-1},t)=f_{(c_1,\ldots, c_{n-1},0), (0,\ldots, 0, 1)}(t)$, which by the assumption of \autoref{lem:localmulti} is a degree-$d$ polynomial. Furthermore, both of these univariate polynomials agree on $d+1$ points, i.e., for every $\beta\in\{0,1,\ldots,d\}$,
        \[ \sum_{e=0}^{d}\delta_{e}(\beta)\cdot f_{e}(c_1,\ldots,c_{n-1}) = \delta_\beta(\beta) \cdot f_\beta(c_1,\ldots, c_{n-1}) = f_\beta(c_1,\ldots, c_{n-1}) = f(c_1,\ldots,c_{n-1},\beta), \]
        When two degree-$d$, univariate polynomials agree on more than $d$ points, they must be identical.
        Thus, we have proven, $\forall \bm{x}\in\mathbb{R}^n$, $f(x_1,\hdots,x_n)=\sum_{e=0}^{d}\delta_{e}(x_n)\cdot f_{e}(x_1,\hdots,x_{n-1})$. Now, $\forall e\in[d]\cup\{0\}$, $deg_{x_{n}}(\delta_e)=d,deg_{x_n}(f_e)=0$, and $\forall i\in[n-1],deg_{x_i}(\delta_e)=0$, and $\sum_{i=1}^{n-1}deg_{x_i}(f_e)=deg(f_e)=d$. So, $$deg(f)=\sum_{i=1}^{n}deg_{x_i}(f)=\max_{e}\left\{deg_{x_n}(\delta_e)+\sum_{i=1}^{n-1}deg_{x_i}(f_e)\right\}=\max_e\{d+d\}=2d.$$ Hence the claim holds.
    \end{proof}
    
    We further bound the degree of $f$ by $d$. We can view $f(x \bm{b})$ as a polynomial $f_{\bm{0},\bm{b}}(x)$ in the formal variables $\bm{b} = (b_1,\ldots, b_n)$, and therefore $f_{\bm{0},\bm{b}}$ has degree $\deg(f)$. \ynote{Why can't we just jump to the second-to-last sentence?} Consider the coefficient $c_{\bm{b}}$ of $x^{\deg(f)}$ in $f(x \bm{b})$. Note that $c_{\bm{b}} \neq 0$, as otherwise $f$ would have degree less than $\deg(f)$. We can view $c_{\bm{b}}$ as a non-zero polynomial in the formal variables $\bm{b}$. Fix any $\bm{b} \in \mathbb{R}^n$ such that $c_{\bm{b}} \neq 0$, then $f_{\bm{0},\bm{b}}(x)$ is a univariate polynomial of degree $\deg(f)$. However, by assumption $f_{\bm{0},\bm{b}}(x)$ has degree at most $d$. Hence, $\deg(f) \leq d$. 
\end{proof}

\paragraph{Proof of \autoref{lem:localuni}.}
%\begin{proof}
    The proof is by induction on the degree of $g$. For any real $t$, we will denote by $D_t[g](x):\mathbb{R}\rightarrow\mathbb{R}$, the discrete derivative operator, applied on $g(x)$, at a step length of $t$, i.e., $D_{t}[g](x)\triangleq g(x+t)-g(x)$. We will use this discrete derivative as a mean of relating degree-$(d-1)$ polynomials to degree-$d$ polynomials. 
    \begin{clm}\label{clm:gg'} For any analytic, univariate function $g:\mathbb{R}\rightarrow\mathbb{R}$ and every $d >1$, $\deg(g)=d$ if and only if $\deg(D_{t}[g])=d-1$, for every $t\in\mathbb{R}\setminus \{0\}$.
    \end{clm}
    \begin{proof}
    $(\Rightarrow)$ Let $g(x)=\sum_{i=0}^{d}c_i x^i$, where $c_d\neq 0$. Then, for all real, non-zero $t$,
    \[
            D_{t}[g](x)=g(x+t)-g(x)=\sum_{i=0}^{d}c_i\left((x+t)^i-x^i\right)=\sum_{i=0}^{d}c_i\left(\sum_{r=0}^{i-1}\binom{i}{r}x^r\cdot t^{i-r}\right).
    \]
    Thus $D_t[g](x)$ has degree $d-1$.
    
     $(\Leftarrow)$ 
    Since $D_t[g](x)$ is a degree-$(d-1)$ polynomial for all  $t\in\mathbb{R}\setminus \{0\}$, we first prove that the derivative $\frac{d}{dx}g\triangleq\lim_{t\rightarrow 0}\frac{D_t[g](x)}{t}$ is a degree-$(d-1)$ polynomial as well: Consider $\frac{D_{t}[g](x)}{t},\forall t\in\mathbb{R}\setminus\{0\}$. They are all degree-$(d-1)$ polynomials (in $x$). From them we define,
    \begin{align*}
        l_1(x) &\triangleq\lim_{t\rightarrow 0^{+}}\frac{D_t[g](x)}{t}=\lim_{t\rightarrow 0^{+}}\frac{g(x+t)-g(x)}{t} \\
        l_2(x) &\triangleq\lim_{t\rightarrow 0^{-}}\frac{D_t[g](x)}{t}=\lim_{t\rightarrow 0^{-}}\frac{g(x+t)-g(x)}{t}=\lim_{t\rightarrow 0^{+}}\frac{g(x-t)-g(x)}{-t}=\lim_{t\rightarrow 0^{+}}\frac{g(x)-g(x-t)}{t}
    \end{align*}
    Since $g$ is analytic, and hence infinitely differentiable, we have $\forall x\in\mathbb{R}, l_1(x)= l_2(x)$. 
    Thus, the derivative $\frac{d}{dx}g$ exists and is equal to $l_1(x)$. 
    Let us now argue that $l_1(x)$ is a degree-$(d-1)$ polynomial. 
    Each element in the sequence $\left\{\frac{D_t[g](x)}{t}\right\}_{t\rightarrow 0^+}$ can be written as $a_{t,d-1}x^{d-1}+\hdots+a_{t,1}x+a_{t,0}$. Each of the sequences $\{a_{t,d-1}\}_{t\rightarrow 0^+},\hdots, \{a_{t,0}\}_{t\rightarrow 0^+}$ is a Cauchy sequence (otherwise, $l_1(x)$ won't exist). Let their limits be $\{a_{t,d-1}\}_{t\rightarrow 0^+}\rightarrow a_{d-1},\hdots, \{a_{t,0}\}_{t\rightarrow 0^+}\rightarrow a_{0}$. Then, $l_1(x)=\lim_{t\rightarrow 0^{+}}\frac{D_t[g](x)}{t}=a_{d-1}x^{d-1}+\hdots+a_{1}x+a_{0}$, is a degree-$(d-1)$ polynomial. Moreover, by single-variable calculus, for $1\leq k \leq d$, $\frac{d^k}{dx^k}g$ is a polynomial of degree 	$d-k$, and $\frac{d^{d+1}}{dx^{d+1}}g = 0$. Hence, by Taylor series expansion:
    \[
    g(x) = \sum_{j = 0}^{d} \frac{1}{j!}\frac{d^j}{dx^j}g(0) \cdot x^j,
    \]
    is a degree-$d$ polynomial.
     %   Let $\forall t,\deg(g'_t)=d-1$, but $\deg(g):=\alpha\neq d$. 
%    Then, we have $g(x)=\sum_{i=0}^{\alpha}c_i x^i$, where $c_{\alpha}\neq 0$, and thus the leading monomial of $g'$ would be $x^{\alpha-1}$, with the coefficient $\alpha c_{\alpha}\neq 0$, making $\deg(g')=\alpha-1\neq d-1$, which is a contradiction.}
    %So, $x^d$ doesn't survive, and the highest surviving exponent of $x$ in $g'(x)$, is $d-1$, as coefficient of $x^{d-1}$ is $d\cdot c_d\neq 0$.
    \end{proof}
    We now resume our proof of \autoref{lem:localuni}, by repeated application of \autoref{clm:gg'}.
    \iffalse By induction on $d$, we will prove that $g$ is a degree-$d$ polynomial if and only if for every $e_1,e_2 \in \mathbb{R}$, $\sum_{i=0}^{d+1} \alpha_i \cdot g(e_1+ie_2) =0$. For the base case ($d=0$), it is easy to see that $g$ has degree $0$. Indeed, $g$ is a constant function, if and only if $\sum_{i=0}^1\alpha_i g(e_1+ie_2)=-g(e_1)+g(e_1+e_2)=0$ for every $e_1,e_2\in\mathbb{R}$.
    
    For the inductive  step, by \autoref{clm:gg'}, $g$ is a degree-$d$ polynomial if and only if $g'_t$ is a degree-$(d-1)$ polynomial for every $t \in \mathbb{R}$. The latter is equivalent to $\sum_{i=0}^{d} \alpha_i  \cdot g'_t(e_1 + ie_2) = 0$ for every $t,e_1,e_2 \in \mathbb{R}$. Hence, $g$ is a degree-$d$ polynomial if and only if for every $e_1,e_2,t \in \mathbb{R}$, 
    \[ \sum_{i=0}^{d} \alpha_i  \cdot \big(g(e_1 + ie_2+t) - g(e_1+i e_2) \big) = 0 \] 
    Setting $t=e_2$ and simplifying: \nnote{we cannot set $t$, as we need to prove it for every $t$}.
    \begin{align*}
            0&=\sum_{i=0}^{d}(-1)^{i+1}\binom{d}{i}\cdot\bigg(g(e_1+ie_2+e_2)-g(e_1+ie_2)\bigg)\\
              &=\sum_{j=1}^{d+1}(-1)^{j}\binom{d}{j-1}\cdot g(e_1+je_2)-\sum_{i=0}^{d}(-1)^{i+1}\binom{d}{i}\cdot g(e_1+ie_2)\\
              &= g(e_1) + (-1)^{d+1} g(e_1 + (d+1)e_2) + \sum_{i=1}^d (-1)^{i}\bigg(\binom{d}{i-1}+\binom{d}{i}\bigg)\cdot g(e_1+ie_2)\\
            &=-\sum_{i=0}^{d+1}(-1)^{i+1}\binom{d+1}{i}\cdot g(e_1+ie_2)=-\sum_{i=0}^{d+1}\alpha_i\cdot g(e_1+ie_2).
    \end{align*}
    where we have used the identity $\binom{d}{i-1}+\binom{d}{i}\ = \binom{d+1}{i}$.\\
    In the forward direction, setting $t=e_2$ is valid, since we only need that set of identities to prove our main identity. In the reverse direction, from $\forall e_1,e_2\in\mathbb{R}, \sum_{i=0}^{d+1}\alpha_i\cdot g(e_1+ie_2)=0$, we get $\forall e_1,e_2\in \mathbb{R}$,$$0=\sum_{i=0}^{d}\alpha_i\cdot g'_{e_2}(e_1+ie_2)=\sum_{i=0}^{d} \alpha_i\bigg(g(e_1+ie_2+e_2)-g(e_1+ie_2)\bigg).$$ In other words: $\forall e_1,e_2\in\mathbb{R},\exists t(=e_2)\in\mathbb{R}:\sum_{i=0}^{d+1}\alpha_i\cdot g'_{t}(e_1+ie_2)=0$. I don't yet see a way to generalize this to $\forall t\in\mathbb{R}$.
    \fi\\
    A univariate (analytic) polynomial $g(x):\mathbb{R}\rightarrow\mathbb{R}$ has degree $d\geq 0\iff\forall t_1,\hdots,t_d\in\mathbb{R}\setminus \{0\},D_{t_d,\hdots,t_1}[g](x)\triangleq D_{t_d}[\hdots[ D_{t_1}[g]]\hdots](x)$ is a degree $0$ polynomial $\iff\forall t_1,\hdots,t_d\in \mathbb{R}\setminus \{0\},\forall e\in\mathbb{R}, D_{t_d,\hdots,t_1}[g](e)=D_{t_d,\hdots,t_1}[g](0)$. Now, we may observe $D_{t_d,\hdots,t_1}[g](x)=D_{t_{d}}[D_{t_{d-1},\hdots,t_1}[g]](x)=D_{t_{d-1},\hdots,t_1}[g](x+t_d)-D_{t_{d-1},\hdots,t_1}[g](x)$. Applying this discrete derivative operator till depth $d$ gives us $$D_{t_d,\hdots,t_1}[g](x)=\sum_{S\subseteq\{t_1,\hdots,t_d\}}(-1)^{|S|}g\Big(x+t_S\Big).$$ Thus, we have the local characterization: $\deg(g)=d$ iff for every $t_1,\hdots,t_d\in\mathbb{R}\setminus \{0\}$ and every $e\in\mathbb{R}$, \[\sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}g\Big(e +t_S \Big)=\sum_{S\subseteq\{t_1,\ldots,t_d\}} (-1)^{|S|}g\Big(t_S\Big). 
    \]\qedhere
    % \hfill \qedsymbol\\
    \iffalse Then, for the inductive step, we have: $deg(g)=d\iff deg(\lim_{t\to 0}g'_{t}(x))=d-1$, which by IH, is equivalent to: $\forall e_1\in\mathbb{R}$,$$0=\lim_{t\to 0}\lim_{\epsilon\to 0}\bigg(\sum_{i=0}^{d}\alpha_i\cdot g'_{t}(e_1+i\epsilon)\bigg)=\lim_{t\to 0}\lim_{\epsilon\to 0}\bigg(\sum_{i=0}^{d}\alpha_i\cdot\big( g(e_1+i\epsilon+t) -g(e_1+i\epsilon)\big)\bigg)$$ Replacing $t,\epsilon$ by a common variable $\nu\to 0$ does the job: we get $\forall e_1\in\mathbb{R}$, 
    \begin{align*}
            0&=\lim_{\nu\to 0}\Bigg[ \sum_{i=0}^{d}(-1)^{i+1}\binom{d}{i}\cdot \bigg(g(e_1+i\nu+\nu)-g(e_1+i\nu)\bigg)\Bigg]\\
              &=\lim_{\nu\to 0}\Bigg[\sum_{j=1}^{d+1}(-1)^{j}\binom{d}{j-1}\cdot g(e_1+j\nu)-\sum_{i=0}^{d}(-1)^{i+1}\binom{d}{i}\cdot g(e_1+i\nu)\Bigg]\\
              &=\lim_{\nu\to 0}\Bigg[ g(e_1) + (-1)^{d+1} g(e_1 + (d+1)\nu) + \sum_{i=1}^d (-1)^{i}\bigg(\binom{d}{i-1}+\binom{d}{i}\bigg)\cdot g(e_1+i\nu)\Bigg]\\
            &=\lim_{\nu\to 0}\Bigg[-\sum_{i=0}^{d+1}(-1)^{i+1}\binom{d+1}{i}\cdot g(e_1+i\nu)\Bigg]=\lim_{\nu\to 0}\Bigg[-\sum_{i=0}^{d+1}\alpha_i\cdot g(e_1+i\nu)\Bigg].
    \end{align*}
    \fi


==> old_deg1_testing.tex <==
\section{Degree-1 testing}

\begin{lem}{(Stability version of the Local to Global for degree $1$-functions)}\label{lem:local_to_global_deg1}
Let $r \in \mathbb{R}^+$ and $F\colon [-r,r]^n\to\mathbb{R}$. If for every line $L$, the restriction of $F$ on the line segment $L\cap [-r,r]^n$ is pointwise $\delta$-close to a univariate  linear function, then there exist a linear function $h\colon \R^n\to\mathbb{R}$ such that $F\colon [-r,r]^n\to\mathbb{R}$ is pointwise $O(n\delta)$-close to $h$ on the hypercube $[-r,r]^n$. 
\end{lem}


\begin{proof}
Let $F^0\colon[-r,r]^n\to\R$ defined as 
\[F^0(\bm x)\triangleq F(\bm x)-F(\bm 0).\]
Note that any line restriction of $F^0$ is close to a linear function. 
We will show that there exists a global linear function $h^0\colon[-r,r]^n\to\R$ such that $h^0$ and $F^0$ are pointwise close in the cube. Then we define $h(\bm x)\triangleq h^0(\bm x)+F(\bm 0)$, to ensure $h$, and $F$ are pointwise close. 
For every $i\in[n]$, define $F_i\colon[-r,r]\to\R$ as 
\[F_i(x)\triangleq F^0(x\bm{e_i}).\]
By assumption, for every $i\in[n]$ there exists a linear function $h_i\colon\R\to \R$ such that for every $x\in [-r,r]$
\[|h_i(x)-F_i(x)|\leq \delta.\]
Let the desired global linear function $h^0:[-r,r]^n\to\R$ be 
\[h^0(\bm x)\triangleq\sum_{i=1}^n h_i(x_i).\]
By definition $h^0$ is linear. 
And for every $\bm x\in [-r,r]^n$ 
\[\left|h^0(\bm x)-F^0(\bm x)\right|\leq \underbrace{\left|\sum_{i=1}^n h_i(x_i)-\sum_{i=1}^n F_i(x_i)\right|}_{\leq n\delta}+\underbrace{\left|\sum_i^n F_i(x_i)-F^0(\bm x)\right|}_{=A}\leq 9n\delta.\]
To show that $A\leq 8n\delta$ we 
use an hybrid sum and rewrite it as:
\begin{align*}
    A=&\left|\sum_{i=1}^n F^0(x_i\bm{e_i})-F^0\left(\sum_{i=1}^n x_i\bm{e_i}\right)\right|\\
    =&\left|\sum_{j=2}^n\left(F^0(x_j\bm{e_j})-F^0\left(\sum_{i=1}^j x_i\bm{e_i}\right)+F^0\left(\sum_{i=1}^{j-1}x_i\bm{e_i}\right)\right)\right|\\
    \leq&\sum_{j=2}^n\left|F^0(x_j\bm{e_j})-F^0\left(\sum_{i=1}^j x_i\bm{e_i}\right)+F^0\left(\sum_{i=1}^{j-1}x_i\bm{e_i}\right)\right|\\
    \leq& 8\delta n.
\end{align*}

The last inequality holds since %the restriction of $F^0$ on any line segment $L_{(\bm x,\bm y)}\cap [-r,r]^n$ is pointwise close to a linear function $h^0$. Therefore 
$F^0$ is $8\delta$-additive, i.e, for every two points $\bm{x,y,x+y}\in[-r,r]^n$ 
\[|F^0(\bm{x+y})-F^0(\bm x)-F^0(\bm y)|\leq 8\delta.\]
Indeed 
\begin{align*}
   |F^0(\bm{x+y})-F^0(\bm x)-F^0(\bm y)|=& |F(\bm{x+y})+F(\bm 0)-F(\bm x)-F(\bm y)|\\
   \leq& \left|F(\bm{x+y})+F(\bm 0)-2F\left(\frac{\bm x+\bm y}{2}\right)\right|+\left|2F\left(\frac{\bm{x+y}}{2}\right)-F(\bm x)-F(\bm y)\right| \\
   \leq& 4\delta+4\delta,
\end{align*}

last inequality is by assumption that $F$, restricted on every line in the cube, is $\delta$-close to a linear function.  




\end{proof}
For degree $=d>1$ case, if we let $S$ to be the set of all degree-$d$ monomials, then $|S|=\binom{n}{d}$. We define $h^0(\bm x)=\sum_{s\in S}h_s(\bm x)/\binom{n-1}{d-1}$, where $s$ denotes a degree-$d$ monomial, and $h_s(\bm x)$ is the degree-$d$ function that is pointwise $\delta$-close to $F_s(\bm x)$, the restriction of $F^0$ on the axis-parallel subspace corresponding to $s$. Let $\bm a_s=(a_{s,1},\hdots, a_{s,n})\in\mathbb F_2^n$ be the indicator vector for this corresponding subspace. Then, for every $\bm x\in[-r,r]^n$,
\begin{align*}
    |h^0(\bm x)-F^0(\bm x)|&\leq\left|\frac{\sum_{s\in S}h_s(\bm x)-\sum_{s\in S}F_s(\bm x)}{\binom{n-1}{d-1}}\right| + \left|\frac{\sum_{s\in S}F_s(\bm x)}{\binom{n-1}{d-1}}-F^0(x_1\bm e_1+\hdots+x_n\bm e_n)\right|\\
    &\leq\frac{\binom{n}{d}\delta}{\binom{n-1}{d-1}} + \left|\frac{1}{\binom{n-1}{d-1}}\sum_{s\in S}F^0\left(\sum_{j=1}^n a_{s,j}x_j\bm e_j\right)-F^0\left(\frac{\sum_{s\in S}\sum_{j=1}^n a_{s,j}x_j\bm e_j}{\binom{n-1}{d-1}}\right)\right|\\
    &\leq\frac{n\delta}{d} + \frac{1}{\binom{n-1}{d-1}}\underbrace{\left|\sum_{s\in S}F^0\left(\sum_{j=1}^n a_{s,j}x_j\bm e_j\right)-\binom{n-1}{d-1}F^0\left(\frac{\sum_{s\in S}\sum_{j=1}^n a_{s,j}x_j\bm e_j}{\binom{n-1}{d-1}}\right)\right|}_{\triangleq A}.
\end{align*}
\begin{align*}
    \sum_{s\in S}F^0\left(\sum_{j=1}^n a_{s,j}x_j\bm e_j\right)&= F^0(\bm 0)(=0)\longleftarrow 0=|s|\triangleq\# x_i\in s\\
    |s|=1\longrightarrow &+F^0(x_1\bm e_1)+F^0(x_2\bm e_2)+\hdots+F^0(x_n\bm e_n)\\
    |s|=2\longrightarrow &+\sum_{i=2}^n F^0(x_1\bm e_1+x_i\bm e_i) +\sum_{i=3}^n F^0(x_2\bm e_2 + x_i\bm e_i)\\
    &+\hdots+\sum_{i=n-1}^n F^0(x_{n-2}\bm e_{n-2}+x_n\bm e_n) + F^0(x_{n-1}\bm e_{n-1} + x_{n}\bm e_n)\\
    |s|=3\longrightarrow &+\sum_{\substack{i,j=2\\ i>j}}^n F^0(x_1\bm e_1+x_i\bm e_i+x_j\bm e_j) + \sum_{\substack{i,j=3\\ i>j}}^n F^0(x_2\bm e_2+x_i\bm e_i+x_j\bm e_j)\\
    &+\hdots+\sum_{\substack{i,j=n-2\\ i>j}}^n F^0(x_{n-3}\bm e_{n-3}+x_i\bm e_i+x_j\bm e_j) + F^0(x_{n-2}\bm e_{n-2}+x_{n-1}\bm e_{n-1}+x_{n}\bm e_{n})\\
    4\leq|s|\leq d-1\longrightarrow &+\vdots+\vdots+\hdots+\vdots\\
    |s|=d\longrightarrow &+ \sum_{\substack{i_1,\hdots,i_{d-1}=2\\ i_1>\hdots>i_{d-1}}}^n F^0(x_1\bm e_1+x_{i_1}\bm e_{i_1}+\hdots+x_{i_{d-1}}\bm e_{i_{d-1}})\\
    &+ \sum_{\substack{i_1,\hdots,i_{d-1}=3\\ i_1>\hdots>i_{d-1}}}^n F^0(x_2\bm e_2+x_{i_1}\bm e_{i_1}+\hdots+x_{i_{d-1}}\bm e_{i_{d-1}})\\
    &+\hdots +\sum_{\substack{i_1,\hdots,i_{d-2}=n-d+1\\ i_1>\hdots>i_{d-2}}}^n F^0(x_{n-d}\bm e_{n-d}+x_{i_1}\bm e_{i_1}+\hdots+x_{i_{d-1}}\bm e_{i_{d-1}})\\
    &+ F^0(x_{n-d+1}\bm e_{n-d+1}+x_{n-d+2}\bm e_{n-d+2}+\hdots+x_{n}\bm e_{n})
\end{align*}

\begin{claim}[conjecture]
Let $g\colon\R^n\to\R$ satisfying $g$ is pointwise $\delta$-close to a univariate degree $d$ function on any line restriction.then $g$ is close to a global function $h\colon\R^n\to\R$ of degree $d$.   
\end{claim}
\begin{proof}
Let 
\[g(x_1,\dots,x_n)=g_0(x_1,\dots,x_{n-1})+x_ng_1(x_1,\dots,x_{n-1}).\]

\end{proof}



==> old_exact.tex <==


Let $d\in\mathbb{N}$.
Given query access to an analytic function $f\colon\mathbb{R}^n\to\mathbb{R}$ and sampling access to $\mathcal{N}(0,I)$, our goal is to design a constant-query (dependent on $d$, independent of the dimension $n$) tester to distinguish between the case where $f$ is a degree-$d$, multivariate polynomial, or $f$ is $\varepsilon$-far from any degree-$d$, multivariate polynomial.
\begin{thm}\label{thm:low_degree_test}
There exists a one-sided error, distribution-free,  $O\left(d^5+\frac{d^2}{\varepsilon}\log\frac{d}{\varepsilon}\right)$-query tester for whether a given analytic function $f\colon\mathbb{R}^n\to\mathbb{R}$ is a degree-$d$ polynomial.
\end{thm}

At a high-level, our tester consists of two steps. First, we test whether $f$ restricted to random lines (sampled from the Gaussian distribution) is consistent with degree-$d$, univariate polynomials on those lines. If $f$ passes this test, then we conclude that there must exist a degree-$d$, polynomial $g\colon\mathbb{R}^n\to\mathbb{R}$ which is a self-corrected version of $f$.
Second, by querying the values of $f$ on a set of correlated points, we are able to get query access to $g$ with high probability, and therefore we can simply estimate the distance between $f$ and $g$. Our tester has one-sided error, i.e., if $f$ is a degree-$d$ polynomial, then our test passes with probability $1$ and furthermore, $g = f$. On the other hand, if $f$ is $\varepsilon$-far from any degree-$d$ polynomial, then our test rejects with high probability. 

Fix $d$ and define $\alpha_i \triangleq (-1)^{i+1}{d+1 \choose i}$.
The self-corrected function $g: \mathbb{R}^n \rightarrow \mathbb{R}$ \ynote{$R$ is undefined} is defined as follows: for every $\bm{p}\in B(\bm{0},R)$, let $g(\bm{p})\triangleq\mathsf{MAJ}_{\bm{q}\sim\mathcal{N}(\bm{0}, I)}\{g_{\bm{q}}(p)\}$, where  $g_{\bm{q}}(\bm{p})\triangleq\sum_{i=1}^{d+1}\alpha_i\cdot f(\bm{p}+i\bm{q})$.
We note that $g_{\bm{q}}(\bm{p})$ is the value of a univariate degree-$d$ polynomial at the point $\bm p$ interpolated by the values $\{f(\bm p+i\bm q)\}_{i=1,\dots,d+1}$.
For $\bm{p}\not\in B(\bm{0},R)$, $g(\bm{p})$ defined as the value of the extension of $g$ as a degree-$d$ polynomial. \ynote{What's the main reason that we first recover $g$ in $B(0,R)$ and then extrapolate it instead of directly recovering $g$ everywhere.}
Formally, to define $g(\bm{p})$ outside $B(\bm{0},R)$, we consider the line $L_{\bm{0},\bm{p}}=\{x\bm{p}\}_{x\in\mathbb{R}}$. 
Since $L_{\bm{0},\bm{p}}$ intersects $B(\bm{0},R)$ and we can show that $g(x\bm{p})$ is a degree-$d$, univariate polynomial inside $B(\bm{0},R)$, we can interpolate $g(x\bm{p})$ by evaluating it on $(d+1)$ distinct points in $B(\bm{0},R)$, obtain the coefficient representation of $g(x\bm{p})$ inside $B(\bm{0},R)$, and then define $g$ for all points on $L_{\bm{0},\bm{p}}$, from this coefficient representation. \nnote{the paragraph about defining $g$ outside of $B$ should be clarified. Probably just state it at a higher level}


\begin{algorithm}[t]
\caption{Distribution-Free Low-Degree Tester}\label{alg:low_degree_main_algorithm}
\Procedure{\emph{\Call{LowDegreeTester}{$f,d,\mathcal{D}$}}}{
  \Given {Query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, degree $d\in\mathbb{N}$, sampling access to the distribution $\mathcal{N}(0, I)$ and sampling access to an unknown distribution $\mathcal{D}$.}
    \textbf{Reject} if \emph{\Call{LocalCharacterizationTest}{$f,d$}} returns \textbf{Reject}\;
   % \textbf{Reject} if \textbf{Test Local Characterization}{($f$)} returns \textbf{Reject}\;
    %\textbf{Reject} if \Call{Force $g^{(t)} = g$.}{f} returns reject\;
    \For{$N_{1} := O(\varepsilon^{-1})$ times}{
      Sample $\bm{p} \sim \mathcal{D}$\;
      \textbf{Reject} if $f(\bm{p}) \neq$ \emph{\Call{Query-$g$}{$\bm{p},f,d$}} or if \emph{\Call{Query-$g$}{$\bm{p},f,d$}} returns \textbf{Reject}.
    }
    \textbf{Accept}.
  }  
\end{algorithm}

\begin{algorithm}[t!]
\caption{Subroutines}\label{alg:subroutines}
\Procedure{\emph{\Call{LocalCharacterizationTest}{$f,d$}}}{
\Given{Query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, degree $d\in\mathbb{N}$, sampling access to the distribution $\mathcal{N}(0, I)$.}
Let $S \triangleq \{i^2 +1 : i \in \{0,\ldots, d+1\} \}$\;
Let $P_1=\{(i^2t,1):i\in[d+1],t\in S\}$ \vnote{$(i,j)$ means an ordered tuple. The way I had defined $t\in S\triangleq\{i^2+1:i\in[d+1]\cup\{0\}\}$, made $|S|=d+2$, so $\#tuples=\#i\cdot|S|=O(d^2)$}  \;
Let $P_2 \triangleq \{(j^2,t):j\in[d+1],t\in S\}$\;
Let $P_3 \triangleq \{(j^2,j^2):j\in[d+1]\}$\;
\For{$N_2 \triangleq O(d^2) $ times }{
\For{$\beta_1,\beta_2\in P_1\cup P_2\cup P_3$}{
      Sample $\bm{p}\sim\mathcal{N}(\bm{0},\beta_1 I),\bm{q}\sim\mathcal{N}(\bm{0},\beta_2 I)$\;
      \textbf{Reject} if $\sum_{i=0}^{d+1}\alpha_i\cdot f(\bm{p}+i\bm{q})\neq 0$\;
    }}
    \textbf{Accept}\;
    }

\Procedure{\emph{\Call{Query-$g$}{$\bm{p},f,d$}}}{
\Given{$\bm{p}\in \mathbb{R}^n$, query access to $f\colon\mathbb{R}^n\to\mathbb{R}$, degree $d\in\mathbb{N}$.}
\If{$\bm{p}\in B(\bm{0},R)$ \ynote{$R$ is undefined}}{
\textbf{return} \emph{\Call{Query-$g$-InSmallBall}{$\bm{p},f,d$}}\;}
Define $\kappa_p \triangleq \frac{R}{(d+1)\Vert \bm{p}\Vert_{2}}$\;

\For{$i\in [d+1]$}{
$g_{(\bm{0,p})}\left({i}{\kappa_p}\right)=$ \emph{\Call{Query-$g$-InSmallBall}{$i\kappa_p\bm{p},f,d$}} or \textbf{Reject} if \emph{\Call{Query-$g$-InSmallBall}{}} returns \textbf{Reject} \;
}
Interpolate a univariate polynomial $g_{(\bm{0},\bm{p})}\colon \mathbb{R}\to\mathbb{R}$ from the  $d+1$ points $\left\{g_{(\bm{0,p})}\left({i}{\kappa_p}\right)\right\}_{i\in [d+1]}$\;
\textbf{return} $g_{(\bm{0,p})}(1)$\;
}

\Procedure{\emph{\Call{Query-$g$-InSmallBall}{$\bm{p},f,d$}}}{
\Given{ $\bm{p}\in B(\bm{0},R(d+1))$, query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, degree $d\in\mathbb{N}$ and sampling access to $\mathcal{N}(0, I)$.}
$N_3  \triangleq O\left(\log\frac{d}{\varepsilon}\right)$\;
Sample $q_1,\dots,q_{N_3}\sim \mathcal{N}(0, I)$\;
\textbf{Reject} if there exists $j\in\set{2,\dots,N_3}$ such that $ \sum_{i=1}^{d+1} \alpha_i \cdot f(\bm{p}+i\bm{q}_1)\neq \sum_{i=1}^{d+1} \alpha_i \cdot f(\bm{p}+i\bm{q}_j)$\;
\textbf{return} $ \sum_{i=1}^{d+1} \alpha_i \cdot f(\bm{p}+i\bm{q}_1)$\;
}
\end{algorithm}



Our algorithm is given in \autoref{alg:low_degree_main_algorithm}, which uses subroutines from \autoref{alg:subroutines}.  The \Call{Query-$g$}{} subroutine  allows us to obtain query access to $g$ with high probability, while the \Call{LocalCharacterizationTest}{$f,d$} subroutine  tests the conditions we require from $f$ in order to prove that $g$ is a degree-$d$ polynomial. 

\begin{lem}
    \label{lem:main_lemma_well_definedness_and_querying_g}
    If \Call{LocalCharacterizationTest}{$f,d$} fails with probability at most $1/16(d+1)(d+2)$, then $g$ is a degree-$d$ polynomial, and furthermore for any $\bm{p}\in\mathbb{R}^n$,  $g(\bm{p})=$ \Call{Query-$g$}{$\bm{p},f$} with probability at least $1-\frac{\varepsilon}{2}$.
\end{lem}

We first prove the main Theorem (\autoref{thm:low_degree_test}) assuming  \autoref{lem:main_lemma_well_definedness_and_querying_g} holds. 
\begin{proof}[{Proof of \autoref{thm:low_degree_test}}]
If $f$ is a degree-$d$ polynomial, then $f$ restricted to a line $\bm{p} + i {\bm q}$ is also a degree-$d$ polynomial. It follows that $g = f$ and each of the tests that the algorithm makes pass with probability $1$.

Now, assume that $f$ is $\varepsilon$-far from any degree-$d$ polynomial. If \Call{LocalCharacterizationTest}{$f,d$} accepts with fails with probability at least $1/16(d+1)(d+2)$, then we reject with probability at least $1-1/16(d+1)(d+2) \geq 2/3$. 
Otherwise, if the test accepts with a higher probability, then by \autoref{lem:main_lemma_well_definedness_and_querying_g} $g$ is a well-defined, degree-$d$ polynomial. Hence, $\delta(f,g)>\varepsilon$ \nnote{define $\delta$}. 
The probability that we do not reject in any of the $N_1$ steps of \autoref{alg:low_degree_main_algorithm} is at most the probability that $f(\bm{p})=g(\bm{p})$ or that  \emph{\Call{Query-$g$}{$\bm{p},f,d$}} returned some value other than $g(\bm{p})$. The latter happens with probability at most $\frac{\varepsilon}{2}$ by \autoref{lem:main_lemma_well_definedness_and_querying_g}. Then, we have
\[\Pr_{\bm{p}\sim \mathcal{D}}[f(\bm{p})=g(\bm{p}) \lor g(\bm{p}) \neq \Call{Query-\mbox{$g$}}{\bm{p},f}]\leq 1-\varepsilon +\frac{\varepsilon}{2}\leq 1-\frac{\varepsilon}{2}.\]
Thus, the probability that \autoref{alg:low_degree_main_algorithm} accepts is at most $\left(1-\frac{\varepsilon}{2}\right)^{N_1}< \frac{1}{3}$ for $N_1$ large enough. 
\end{proof}

In the remainder of this section we will prove \autoref{lem:main_lemma_well_definedness_and_querying_g}.
\nnote{In general the next section needs more exposition. For example, why are we using this line restriction function. Perhaps moving it earlier would be good. i.e., have a section where we outline the criterion we will test for being a degree $d$ polynomial.}
We will sample vectors $\bm{p},\bm{q} ~\sim \mathcal{N}(0,I)$ and look at the function $f$ restricted to the line $L_{\bm p,\bm{q}}$ defined as $f_{\bm{p},\bm{q}}(x) \triangleq f(\bm{p}+x\bm{q})$. 

\nnote{the next paragraph probably goes in the intro}
Finite forward differences and derivatives are related, i.e., for all differentiable functions $g,D_{h}[g](x)=\frac{\Delta_h[g](x)}{h}+O(h)$ \nnote{Explain further, or give a citation}. In \emph{\Call{LocalCharacterizationTest}{}} we indirectly test if $\Delta_h^{(d+1)}[f_{\bm{p},\bm{q}}](x) =  0$, for small $h$, by testing if $\sum_{i=0}^{d+1}\alpha_{i}f(\bm{p}+i\bm{q})=0$, where $\bm{p},\bm{q}\sim\frac{\sum_{j=1}^{d+1}\mathcal{N}(\bm{0},jI)}{d+1}$.

We record several observations which will be useful throughout the rest of the proof. \nnote{In general I found these observations difficult to read. It might be helpful to state them and then prove them in the proof environment} 
\begin{obs}\label{obs:form-of-diff}
$\Delta_h^{(d+1)}[f_{\bm{p},\bm{q}}](x)=(-1)^d\sum_{i=0}^{d+1}\alpha_i\cdot f(\bm{p}+x\bm{q}+ih\bm{q})$.
\end{obs}
\begin{proof}
  $\Delta_h^{(d+1)}[f_{\bm{p},\bm{q}}](x)=\sum_{i=0}^{d+1}(-1)^{d+1-i}\binom{d+1}{i}f_{\bm{p},\bm{q}}(x+ih)=(-1)^d\sum_{i=0}^{d+1}\alpha_i\cdot f(\bm{p}+x\bm{q}+ih\bm{q})$.  
\end{proof}
\begin{obs}\label{obs:random-vec-choice-suff} 
For testing $\Delta_h^{(d+1)}[f_{\bm{a},\bm{b}}](x)=0$, the sequence $\{\underbrace{\bm{a}+x\bm{b}}_{\bm{p}}+i\underbrace{h\bm{b}}_{\bm{q}}\}_{i=0}^{d+1}$ of points suffices.  \ynote{What does it mean by ``suffice''}
\end{obs}
\begin{obs}\label{obs:one-sided-tester}
If $f_{\bm p, \bm q}$ is a degree-$d$ univariate polynomial, then \ynote{broken sentence}
When $\lim_{h\rightarrow 0}D_{h\cdot\bm{1}}[f_{\bm{p},\bm{q}}](x) = 0= \lim_{h\rightarrow 0}\frac{\Delta_h^{(d+1)}[f_{\bm{p},\bm{q}}](x)}{h^{d+1}}$, making our tester a one-sided error tester. \nnote{Should expand upon why it makes it a one sided tester}
 So, $D_{h\cdot\bm{1}}[g](x)=\sum_{i=0}^{d+1}\alpha_i\cdot g(x+ih)$, for $\bm{1}=(1,1,\hdots,1)\in\mathbb{R}^{d+1}$. 
\end{obs}
\begin{proof}

\end{proof}
On the other hand, the following holds.
\begin{obs}\label{obs:finite-diff-test-suffices}
Let $\bm p, \bm q \in \mathbb{R}^n$ and $f: \mathbb{R}^n \rightarrow \mathbb{R}$ be any analytic function. If $\lim_{h\rightarrow 0}\Delta_{h}^{(d+1)}[f_{\bm p,\bm q}](x)=0$, then $\lim_{h\rightarrow 0}D_{h\cdot\bm{1}}[f_{\bm{p},\bm{q}}](x)=0$.
%\[ \lim_{h\rightarrow 0}D_{h\cdot\bm{1}}[f_{\bm{p},\bm{q}}](x)=\lim_{h\rightarrow 0}\left(\frac{\Delta_h^{(d+1)}[f_{\bm{p},\bm{q}}](x)}{h^{d+1}}+O(h)\right) = 0, \] 
%and $f_{\bm p,q} \in \mathcal{P}_d$. 
%$$\lim_{h\rightarrow 0}D_{h\cdot\bm{1}}[f_{\bm{p},\bm{q}}](x)=\lim_{h\rightarrow 0}\left(\frac{\Delta_h^{(d+1)}[f_{\bm{p},\bm{q}}](x)}{h^{d+1}}+O(h)\right)=\lim_{h\rightarrow 0}O(h)=0.\implies f_{\bm{p},\bm{q}}\in\mathcal{P}_d,$$
\end{obs}
\begin{proof}
Let ${\bm t} \in \mathbb{R}^d$ be any vector. We claim that we can assume ${\bm t} = h \cdot \bm{1}$ for any $h \in \mathbb{R}$. Indeed,
\begin{align*}
    \lim_{\bm{t}\rightarrow\bm{0}}D_{\bm{t}}[f_{\bm p,q}](x) &= \lim_{(\bm{t}_{1},\ldots, \bm{t}_{d-1})\rightarrow\bm{0}}D_{(\bm{t}_{1},\ldots, \bm{t}_{d-1})}\left[\lim_{t_d\rightarrow 0}D_{\bm{t}_d}[f_{\bm{p},\bm{q}}]\right](x) \\
    &=  \lim_{(\bm{t}_{1},\ldots, \bm{t}_{d-1})\rightarrow \bm{0}}D_{(\bm{t}_{1},\ldots, \bm{t}_{d-1})}\left[\lim_{h\rightarrow 0}D_{h}[f_{\bm{p},\bm{q}}]\right](x).
\end{align*}
Repeating this process for each ${\bm t}_i$, we have $\lim_{\bm{t}\rightarrow \bm{0}}D_{\bm{t}}[f_{\bm p,\bm q}](x) = \lim_{h\rightarrow 0}D_{h \cdot \bm{1}}[f_{\bm p,\bm q}](x)$. Now, by assumption we have that
\[ \lim_{h\rightarrow 0}D_{h\cdot\bm{1}}[f_{\bm{p},\bm{q}}](x)=\lim_{h\rightarrow 0}\left(\frac{\Delta_h^{(d+1)}[f_{\bm{p},\bm{q}}](x)}{h^{d+1}}+O(h)\right) = \lim_{h \rightarrow 0} O(h) = 0.\] 


\nnote{Why does this complete the proof of the claim? We need to cite some lemma here (\autoref{thm:Usefulchar}).}
%since \nnote{$t_d$ be the first $d$ points of the vector, $t_{d-1}$ first $d-1$ points. $\rightarrow d$ means taking $d$ steps}
%$$\lim_{\bm{t_d}\rightarrow 0}D_{\bm{t_d}}[f_{\bm{p},\bm{q}}](x)=\lim_{\bm{t_{d-1}}\rightarrow 0}D_{\bm{t_{d-1}}}\left[\lim_{t_d\rightarrow 0}D_{t_d}[f_{\bm{p},\bm{q}}]\right](x)=\lim_{\bm{t_{d-1}}\rightarrow 0}D_{\bm{t_{d-1}}}\left[\lim_{h\rightarrow 0}D_{h}[f_{\bm{p},\bm{q}}]\right](x)\xrightarrow{d}\lim_{h\rightarrow 0}D_{h\cdot\bm{1}}[f_{\bm{p},\bm{q}}](x).$$ \nnote{This seems to be where we prove our characterization of degree $d$ polynomials holds. This should be in its own lemma. It also might be good to use a different function rather than $g$ when defining the iterated derivative operator, unless you really mean the self-corrected function $g$. I also do not follow the proof. Here's some things I didn't understand: What are $\bm t_d, t_{d-1}$? Why is the first equality true? What is meant by $\xrightarrow{d}$?}
\end{proof}

%The self corrected function $g$ is defined as $g(\bm{p})=\mathsf{MAJ}_{t\in[(d+2)^2]}\{g^{(t)}(\bm{p})\}\text{, where }g^{(t)}(\bm{p})=\mathsf{MAJ}_{\bm{q}\sim\mathcal{N}(\bm{0}, tI)}\{g_{\bm{q}}(p)\}$, and $g_{\bm{q}}(\bm{p})=\sum_{i=1}^{d+1}\alpha_i\cdot f(\bm{p}+i\bm{q})$. 




\iffalse{}
If the modified small ball characterization holds \nnote{What is the modified small ball characterization?}, then $g$ is a degree $d$ multivariate polynomial inside $B(\bm{0},R)$. This gives a coefficient representation for $g(\bm{x})=\sum_{\bm{\alpha}:\|\bm{\alpha}\|_1\leq d}c_{\bm{\alpha}}\cdot\bm{x}^{\bm{\alpha}}$. All restrictions $g(x\bm{p})$ agree with this coefficient representation inside $B(\bm{0},R)$, and thus $Q_{\bm{p}}(x)$ defined by interpolation of $g(x\bm{p})$ agree on points outside $B(\bm{0},R)$ as well \nnote{What does $Q_p(x)$ agree with? Might also be good to formally define $Q_p$}.
\fi


%Alternatively, we define the restrictions of $g$ to planes passing through the origin, $g_{P(\bm{a},\bm{b})}(x,y)=g(x\bm{a}+y\bm{b}):\mathbb{R}^2\rightarrow\mathbb{R}$, and we prove these restrictions are all degree-$d$, bivariate polynomials.
%Then, any line restrictions of $g$, defined as restrictions of these plane restrictions will be automatically degree-$d$, univariate polynomials. 
%We observe any line $L_{\bm{u},\bm{v}}=\{\bm{u}+x\bm{v}\}_{x\in\mathbb{R}}$, and the origin, define a plane $P(L_{\bm{u},\bm{v}})$ passing through the origin. So, if all such plane restrictions of $g$ are degree $d$, bivariate polynomials, then all line restrictions of $g$ will be degree $d$, univariate polynomials, making $G$, a degree $d$, multivariate polynomial. So, we randomly sample $\bm{p},\bm{q}$, and test if $g(x\bm{p}+y\bm{q})$ is a deg $d$, bivariate poly, by testing its $(d+1)^{th}$-order finite differences w.r.t both $x,y$ are identically zero.

==> old_exact_tester_code.tex <==

\Procedure{\emph{\Call{LocalCharacterizationTest}{$f,d$}}}{
\Given{Query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, degree $d\in\mathbb{N}$, sampling access to the distribution $\mathcal{N}(0, I)$.}
\For{$N_2 \triangleq O(d^2) $ times}{
Sample $\bm{p_1,p_2},\bm{q_1,q_2}\sim\mathcal{N}(\bm{0}, I)$ \;
\For{$i=1,\dots, d+1$}{
      \textbf{Reject} if $\sum_{k=0}^{d+1}\alpha_k\cdot f(i\bm{p_1}+k(i\bm{q_1}))\neq 0$\;
\For{$j=0,\dots,d+1$}{
      \textbf{Reject} if $\sum_{k=0}^{d+1}\alpha_k\cdot f(i\bm{p_1}+k(\bm{q_1}+j\bm{q_2}))\neq 0$\;
      \textbf{Reject} if $\sum_{k=0}^{d+1}\alpha_k\cdot f((i\bm{p_1}+ij\bm{p_2})+k\bm{q_1})\neq 0$\;
    }}}
    \textbf{Accept}\;
    }
    
    
 
\Procedure{\emph{\Call{LocalCharacterizationTest}{$f,d$}}}{
\Given{Query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, degree $d\in\mathbb{N}$, sampling access to the distribution $\mathcal{N}(0, I)$.}
\For{$N_2 \triangleq O(d^2) $ times}{
\For{$i=1,\dots, d+1$}{
Sample $\bm{p},\bm{q}\sim\mathcal{N}(\bm{0}, i^2I)$ \;
      \textbf{Reject} if $\sum_{k=0}^{d+1}\alpha_k\cdot f(\bm{p}+k\bm{q})\neq 0$\;
\For{$j=0,\dots,d+1$}{
      Sample $\bm{p}\sim\mathcal{N}(\bm{0},i^2I),\bm{q}\sim\mathcal{N}(\bm{0},(j^2+1)I)$ \;
      \textbf{Reject} if $\sum_{k=0}^{d+1}\alpha_k\cdot f(\bm{p}+k \bm{q})\neq 0$\;
      Sample $\bm{p}\sim\mathcal{N}(\bm{0},(i^2(j^2+1)I),\bm{q}\sim\mathcal{N}(\bm{0},I)$ \;
      \textbf{Reject} if $\sum_{k=0}^{d+1}\alpha_k\cdot f(\bm p+k\bm{q})\neq 0$\;
    }}}
    \textbf{Accept}\;
    }
       
\end{algorithm}


==> tolerant.tex <==
%!TEX root=./main.tex

\section{Tolerant Testing}

\subsection{Sketch}

Given input function $f: \R^n \to \R$, we want to distinguish between following two cases with probability $2/3$:
\begin{itemize}
\item
(YES case) There exists a degree-$d$ polynomial $h: \R^n \to \R$ such that for all $\bm{p} \in \R^n$:
\[
|f(\bm{p})-h(\bm{p})| < \eps_1;
\]
\item
(NO case)\footnote{We can also look at $\ell_1$-norm instead of $\ell_2$-norm here.} For any degree-$d$ polynomial $h: \R^n \to \R$:
\[
\Exp_{\bm{p} \sim \cN(0,I)}[|f(\bm{p})-h(\bm{p})|^2] > \eps_2^2.
\]
\end{itemize}
\ynote{This is a non-standard definition. Usually we want to distinguish the case $\delta(f,h) < \epsilon_1$ from the case $\delta(f,h) > \epsilon_2$, where $\delta(f,h) = \Pr_{x \sim \mathcal{D}}[f(x) \neq g(x)]$.}

Here is our current plan:

\begin{itemize}
\item
Define $g(p)$ as the median over $\bm{q} \sim \cN(0,I)$ of $g_{\bm{q}}(\bm{p})$ instead of the majority as earlier.

\item
Observe that
\[
\Pr_{\bm{q}_1, \bm{q}_2}[|g_{\bm{q}_1}(\bm{p}) - g_{\bm{q}_2}(\bm{p})| <\delta] > 1-\eta
\]
implies
\[
\Pr_{\bm{q}_1}[|g_{\bm{q}_1}(\bm{p}) - g(\bm{p})| <\delta] > 1-2\eta.
\]

\item
We then use Lemma \ref{lem:noisy-collision} (or something similar) to get a bound on $\eta$.

\item
We then extend Theorem \ref{thm:characterization_in_small_ball} to get an a bound on $\sum_{i=0}^{d+1}\alpha_i\cdot g(\bm{p}+i\bm{q})$ 
for small enough $\bm{p}$ and $\bm{q}$. 

\item
\textcolor{red}{MAIN QUESTION:} What does a bound on $\sum_{i=0}^{d+1}\alpha_i\cdot g(\bm{p}+i\bm{q})$  imply about
\[
\inf_h \Exp_{\bm{p} \sim \cN(0,I)}[|g(\bm{p})-h(\bm{p})|^2]
\]
where the infimum is over degree-$d$ polynomials $h$?
\end{itemize}



\subsection{Notes}
If we modify \Call{CharacterizationTest}{$f,d$} to reject if $\sum_{i=0}^{d+1}|\alpha_i\cdot f(\bm{p}+i\bm{q}_1)|>2^d\epsilon_1$, and define $g(\bm{p})=\mathbb{E}_{\bm{q}}\{g_{\bm{q}}(\bm{p})\}$, where $g_{\bm{q}}(\bm{p})=\sum_{i=1}^{d+1}\alpha_i\cdot f(\bm{p}+i\bm{q})$, then modified Lemma~\ref{lem:well_defined_of_g} reads as:
\begin{lem}\label{lem:noisy-collision}
$\forall\bm{p}\in B(\bm{0},R),\forall s,t\in[(d+2)^2]$,
$$\Pr_{\substack{\bm{q}_1\sim\mathcal{N}(\bm{0},sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|>2^{d+1}(d+1)\epsilon_1]\leq\sigma=(d+1)(2\rho+(d+2)(2d+3)(s+t)R/6).$$
\end{lem}
\begin{proof}
We have $g_{\bm{q}_1}(\bm{p})=\sum_{i=1}^{d+1}\alpha_i\cdot f(\bm{p}+i\bm{q}_1),g_{\bm{q}_2}(\bm{p})=\sum_{i=1}^{d+1}\alpha_i\cdot f(\bm{p}+i\bm{q}_2)$. For any fixed $i\in[d+1]$,
\begin{equation*}
\begin{split}
    &\Pr_{\substack{\bm{q}_1\sim\mathcal{N}(\bm{0},sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}}\left[|f(\underbrace{\bm{p}+i\bm{q}_1}_{\triangleq\bm{r}})-g_{\bm{q}_2}(\bm{p}+i\bm{q}_1)|>2^d\epsilon_1\right]=\Pr_{\substack{\bm{r}\sim\mathcal{N}(\bm{p},i^2sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}}\left[\left|f(\bm{r})-\sum_{j=1}^{d+1}\alpha_j\cdot f(\bm{r}+j\bm{q}_2)\right|>2^d\epsilon_1\right]\\
    &\leq\underbrace{\Pr_{\substack{\bm{r}\sim\mathcal{N}(\bm{0},i^2sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}}\left[\left|\sum_{j=0}^{d+1}\alpha_j\cdot f(\bm{r}+j\bm{q}_2)\right|>2^d\epsilon_1\right]}_{\leq\rho}+2\underbrace{d_{TV}\left(\mathcal{N}(\bm{0},i^2sI),\mathcal{N}(\bm{p},i^2sI)\right)}_{\leq i^2sR/2}\leq\rho+i^2sR.
\end{split}
\end{equation*}
Similarly, for any fixed $j\in[d+1]$,
$$\Pr_{\substack{\bm{q}_1\sim\mathcal{N}(\bm{0},sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}}\left[|f(\bm{p}+j\bm{q}_2)-g_{\bm{q}_1}(\bm{p}+j\bm{q}_2)|>2^d\epsilon_1\right]\leq\rho+j^2tR.$$
Taking a union bound over $i,j\in[d+1]$, we get
\begin{equation*}
\begin{split}
    \Pr_{\substack{\bm{q}_1\sim\mathcal{N}(\bm{0},sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}} \Bigg[\Big| \underbrace{\sum_{i=1}^{d+1} \alpha_i  \cdot f(\bm{p}+i\bm{q}_1)}_{=g_{\bm{q}_1}(\bm{p})}- \sum_{i=1}^{d+1} \sum_{j=1}^{d+1} \alpha_i \alpha_j  \cdot f((\bm{p}+i\bm{q}_1) + j\bm{q}_2)\Big|>2^d(d+1)\epsilon_1 \Bigg] \leq (d+1)\rho +\sum_{i=1}^{d+1}i^2sR,\\
    \Pr_{\substack{\bm{q}_1\sim\mathcal{N}(\bm{0},sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}} \Bigg[\Big| \underbrace{\sum_{j=1}^{d+1} \alpha_j  \cdot f(\bm{p}+j\bm{q}_2)}_{=g_{\bm{q}_2}(\bm{p})}- \sum_{j=1}^{d+1} \sum_{i=1}^{d+1} \alpha_j \alpha_i  \cdot f((\bm{p}+j\bm{q}_2) + i\bm{q}_1)\Big|>2^d(d+1)\epsilon_1 \Bigg] \leq (d+1)\rho +\sum_{j=1}^{d+1}j^2tR.
\end{split}
\end{equation*}
Another union bound over these gives us
$$\Pr_{\substack{\bm{q}_1\sim\mathcal{N}(\bm{0},sI)\\ \bm{q}_2\sim\mathcal{N}(\bm{0},tI)}}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|>2^{d+1}(d+1)\epsilon_1]\leq\underbrace{(d+1)(2\rho+(d+2)(2d+3)(s+t)R/6)}_{\triangleq\sigma}.$$
\end{proof}

\section{Testing Polynomials with Noise - Alternative Definition}

Given input function $f: \R^n \to \R$, we want to distinguish between following two cases with probability $2/3$:
\begin{itemize}
\item
(YES case) There exists a degree-$d$ polynomial $h: \R^n \to \R$ such that for all $\bm{p} \in \R^n$:
\[
|f(\bm{p})-h(\bm{p})| < \delta;
\]
\item
(NO case) For any degree-$d$ polynomial $h: \R^n \to \R$:
\[
\Pr_{\bm{p} \sim \cN(0,I)}[|f(\bm{p})-h(\bm{p})|>2\delta] > \eps.
\]
\end{itemize}



\subsection{Degree-$1$ Univariate Polynomials}

Let $0<a\in \R$ large enough constant (depends on $\varepsilon$) such that 
\[\Pr_{x\sim\cN(0,1)}[x\not\in[-a,a]]\leq \frac{\varepsilon}{2}.\]


\begin{algorithm}[t!]
\caption{Degree-$1$ Univariate Tester}\label{alg:degree_1_univariate}
\Procedure{\emph{\Call{ApproximateLineTester}{$f$}}}{
  \Given {Query access to $f\colon \mathbb{R} \rightarrow \mathbb{R}$, sampling access to the Gaussian distribution $\mathcal{N}(0, 1)$.}
  $\tilde{h}\colon[-a,a]\to\R :=$ be the interpolation of the line passes through the points $(-a,f(-a)),(a,f(a))$\;
  \For{$N := O(\varepsilon^{-1})$ times}{
      Sample $x \sim \mathcal \cN(0,1)$\;
      \If{$x\in[-a,a]$}
      {\textbf{Reject} if $|f(x)-\tilde{h}(x)|\geq 2\delta$\;}
    }
    \textbf{Accept}.
  }  
\end{algorithm}


\begin{thm}{(Univariate degree-$1$ tester with noise)}\label{thm:univariate_degree1_with_noise}

There exists a one-sided error $O\left(\frac{1}{\varepsilon}\right)$-query tester for degree-$1$ functions $f\colon\R\to\R$ over the standard Normal distribution, in the presence of bounded noise. 


\end{thm}

\begin{proof}

Our tester is given in Algorithm \ref{alg:low_degree_main_algorithm}, which defines a degree-$1$ polynomial $\tilde{h}$ on the  range $[-a,a]$ where most of the samples mass is. 
$\tilde{h}$ take the line that passes between the two endpoints $(-a,f(-a))$ and $(a,f(a))$. 
The slop of $\tilde{h}$ is $\frac{f(a)-f(-a)}{2a}$,
and its  y-intercept  is 
$\frac{f(-a)+f(a)}{2}$.

%Therefore $\tilde{h}(x)=\frac{f(a)-f(-a)}{2a}x+\frac{f(-a)+f(a)}{2}$. 
\paragraph{Soundness:}
 In the NO case, $f$ is $\varepsilon$ far from every line and particularly $f$ is far from $\tilde{h}$, the points outside $[-a,a]$ are samples with probability at most $\frac{\varepsilon}{2}$ and therefore, with probability $\frac{\varepsilon}{2}$ points in $[-a,a]$ are far from $\tilde{h}$. Choosing $N$ to be large enough, one of these witnesses will be caught by Algorithm \ref{alg:degree_1_univariate}, with high probability, in this case the tester rejects.
 \paragraph{Completeness:}
We will show that for the YES case $\tilde{h}$ is $2\delta$ close to $f$ for every point in $[-a,a]$ and therefore Algorithm \ref{alg:degree_1_univariate} never reject, thus, we have a perfect completeness.  


\begin{claim}
 Let $f\colon\R\to\R$ be a $\delta$-noisy version of a degree-$1$ univariate polynomial $h\colon\R\to\R$. i.e, For all $x\in \R$, $|f(x)-h(x)|\leq \delta$.
 And Let $\tilde{h}\colon[-a,a]\to\R$ be defined as 
 \[\tilde{h}=\frac{f(a)-f(-a)}{2a}x+\frac{f(-a)+f(a)}{2}.\]
 Then for every $x\in[-a,a]$, $|f(x)-\tilde{h}(x)|\leq 2\delta.$ 
\end{claim}
 
 \begin{proof}
 Let $h(x)=mx+b$ for some $m,b\in\R$. 
 Then $f(-a)=h(-a)+\delta_{-a}=m(-a)+b+\delta_{-a}$ and  $f(a)=ma+b+\delta_a$ for some $\delta_{-a},\delta_a\in [-\delta,\delta]$. 
 Now, we can rewrite 
 \[\tilde{h}(x)=\frac{(ma+b+\delta_a)-(m(-a)+b+\delta_{-a})}{2a}x+\frac{(m(-a)+b+\delta_{-a})+(ma+b+\delta_a)}{2}.\]
 \[\tilde{h}(x)=mx+\frac{\delta_a-\delta_{-a}}{2a}x+b+\frac{\delta_{-a}+\delta_a}{2}=mx+b+\delta_{-a}\frac{a-x}{2a}+\delta_a\left(1-\frac{a-x}{2a}\right).\]
 
 For every $x\in [-a,a]$
 \[|f(x)-\tilde{h}(x)|\leq |f(x)-h(x)|+|h(x)-\tilde{h}(x)|\leq \delta+\left|\delta_{-a}\frac{a-x}{2a}+\delta_a\left(1-\frac{a-x}{2a}\right)\right|\leq 2\delta.\]
 Last inequality is since $-a\leq x\leq a$ we have $0\leq\frac{a-x}{2a}\leq 1$ and both $|\delta_{-a}|$ and $|\delta_a|$ are at most $\delta$.
 \end{proof}
 
 \end{proof}
 
 \subsection{Plan for Degree-$1$ multivariate polynomials}
 
 \paragraph{Local characterization}
 Sample $\bm{p,q}\sim\cN(0,I)$. 
 Reject if $f(\bm{p})$ is $\delta$-far from the line defined by 2 endpoints of the line $L_{\bm{p,q}}$ intersect a reasonable cube (of large enough constant side length) (or a ball).  


Define $g_{\bm{q}}(\bm{p})=\tilde{h}_{\bm{p,q}}(\bm{p})$.
And $g(\bm{p})=Median_{\bm{q}}[g_{\bm{q}}(\bm{p})]$

Show that $g$ on every line is $\delta$-close to degree-$1$ unvariate polinomial. 

Show local to global theorem for the noisy version --- use discretization to find the best one? 

Choose $O\left(\frac{1}{\varepsilon}\right)$ random points $\bm{p}\sim\cN(0,I)$ and reject if they are $2\delta$-far from QUERY-$g(\bm{p})$.

Where QUERY-$g(\bm{p})$ take the Madian of $g_{\bm{q}}(\bm{p})$ out of enough sampled $\bm{q}$.










\subsection{Local to Global with Noise}

\begin{lem}{(Local to Global)}\label{lem:local_to_global}
Let $r \in \mathbb{R}^+$ and $F\colon [-r,r]^n\to\mathbb{R}$. If for every $\bm{a}\in [-r,r]^n,i\in [n]$. The restriction of $F$ on the line segment $L_{\bm{a},\bm{e_i}}\cap [-r,r]^n$ --- the function $F_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$ is point-wise $\delta$-close to a univariate  degree-$d$ polynomial $h_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$, then $F\colon [-r,r]^n\to\mathbb{R}$ is point-wise close to  a multivariate polynomial $h\colon [-r,r]^n\to\mathbb{R}$ which is of degree at most $nd$. 
\end{lem}
\begin{proof}

We show that $F$ is close to a bounded degree ($nd$) polynomial  by induction on the dimension $n$. For the base case when $n=1$, we have that $F=F_{(0,1)}$ and therefore close to a degree-$d$ polynomial by assumption. 

Now, assume the statement is true for dimension $n-1$. 
Let $c\in[-r,r]$ and define $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ as
\[F_c(a_1,\dots,a_{n-1}):=F(a_1,\dots,a_{n-1},c).\]
We will argue that $F_c$ is close to a degree-$(n-1)d$ polynomial $h_c$. 
Fix some $\bm{a}\in[-r,r]^{n-1}$ and define $\bm a^\uparrow=(a_1,\dots,a_{n-1},c) \in [-r,r]^n$ to be an extension of $\bm a$ to dimension $n$. As well, for $i\in [n-1]$, let $\bm e_i \in \{0,1\}^n$ and $\bm e_i^\uparrow \in \{0,1\}^n$ be the $i$th standard basis vectors in dimension $n-1$ and $n$ respectively. By assumption, $F_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$ is close to a degree-$d$ polynomial $h_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$. Now, for every $x\in[-r-a_i,r-a_i]$ we have
\[F_{\bm a^\uparrow, \bm e_i^\uparrow}(x)=F(a_1,\dots,a_{i-1},a_i+x,a_{i+1},\dots,a_{n-1},c)=F_c(\bm{a}+x\bm{e_i})=(F_c)_{\bm{a,e_i}}(x).\]
Thus, $(F_c)_{\bm{a,e_i}}(x)$ is close to a degree-$d$ polynomial 
%denoted by $(h_c)_{\bm{a,e_i}}(x)$$
on the domain $[-r-a_i,r-a_i]$. Thus, by the inductive hypothesis we can conclude that $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ is close to a degree-$(n-1)d$ multivariate polynomial $h_c\colon[-r,r]^{n-1}\to\mathbb{R}$. 
 
It remains to show that $F$ is close to a degree-$nd$ polynomial $h$. Let $c_0,c_1,\dots, c_d\in[-r,r]$ be any $d+1$ distinct values. Using these $d+1$ points, for every $i\in\{0,\dots,d\}$ we define the degree-$d$ polynomial $\delta_{c_i}$ defined uniquely by its evaluation on these $d+1$ points, so that \[\delta_{c_i}(c_j)=\begin{cases}1 & i=j,\\0 &i\neq j.\end{cases}\] 
% Since any degree-$d$ polynomial is defined uniquely by $d+1$ points, for $t \neq c_j$ for all $j$, $\delta_{c_i}(t)$ is well-defined. 
 Using $\delta_{c_i}$, we will show that $h\colon[-r,r]^{n}\to\mathbb{R}$ can be written as a polynomial of degree $nd$.
% \[F(x_1,\dots,x_n)=\sum_{i=0}^{d}\underbrace{\delta_{c_i}(x_n)}_{degree- d}\underbrace{f_{c_i}(x_1,\dots,x_{n-1})}_{degree-(n-1)d}.\]






Define
 \[h(x_1,\dots,x_n)\equiv\sum_{i=0}^{d}\underbrace{\delta_{c_i}(x_n)}_{degree- d}\underbrace{h_{c_i}(x_1,\dots,x_{n-1})}_{degree-(n-1)d},\]
$h$ is degree $nd$ as it defined. It left to show that $h$ and $F$ are point-wise close on the domain $[-r,r]^n$. 

We claim that for every $\bm{a}\in [-r,r]^{n-1}$ and formal variable $t$,
$h_{\bm a}(t)=h(a_1,\dots,a_{n-1},t)$ is degree $d$ as its defined.
Moreover, it close to $F_{(\bm a,0),\bm{e_n}}$ on the points $t=c_0,\dots, c_d$, while by the assumption $F_{(\bm a,0),\bm{e_n}}$ is close to some univariate degree-$d$ function $\tilde{h}$, therefore for every $i\in\{0,\dots,d\}$ we have 
\[|h_{\bm a}(c_i)-\tilde{h}(c_i)|\leq 2\delta.\]

We have to show that this imply that for every $x$ in the cube $|h_{\bm a}(x)-\tilde{h}(x)|\leq 2\delta.$
\enote{Here I stuck with the proof}.\vnote{Noah, and I discussed this, and were inconclusive if this is true. A line of thought: Consider the zeroes of $h_{\bm{a}}(x)-\tilde{h}(x)$. They have to be countable, because if the measure of zeroes of an analytic function $f(=h_{\bm{a}}-\tilde{h})$ is non-zero, then $f\equiv 0$. An example is $h_{\bm{a}}(x)=\tilde{h}(x)+\delta\sin{\pi  x}$. Here $f(x)=0,\forall x\in\mathbb{Z},f\not\equiv 0$, and $|f|\leq\delta$. If the set of zeroes were finite, then consider the largest zero $x_0$. For all $x>x_0,|f(x)|>0$, and $f(x)$ doesn't change sign}
\end{proof}

\paragraph{Linearity Testing (degree-$1$ polynomials)}

\begin{lem}{(Local to Global)}\label{lem:local_to_global}
Let $r \in \mathbb{R}^+$ and $F\colon [-r,r]^n\to\mathbb{R}$. If for every $\bm{a}\in [-r,r]^n,i\in [n]$. The restriction of $F$ on the line segment $L_{\bm{a},\bm{e_i}}\cap [-r,r]^n$ --- the function $F_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$ is point-wise $\delta$-close to a univariate  linear function $h_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$, then $F\colon [-r,r]^n\to\mathbb{R}$ is point-wise $2n\delta$-close to  a multi-linear polynomial $h\colon [-r,r]^n\to\mathbb{R}$. 
\end{lem}
\begin{proof}

We show that $F$ is $2n\delta$-close to a multi-linear polynomial by induction on the dimension $n$. For the base case when $n=1$, we have that $F=F_{(0,1)}$ and therefore is $\delta$-close to a linear function by assumption. 

Now, assume the statement is true for dimension $n-1$. 
Let $c\in[-r,r]$ and define $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ as
\[F_c(a_1,\dots,a_{n-1}):=F(a_1,\dots,a_{n-1},c).\]
We will argue that $F_c$ is close to a multi-linear function $h_c$. 
Fix some $\bm{a}\in[-r,r]^{n-1}$ and define $\bm a^\uparrow=(a_1,\dots,a_{n-1},c) \in [-r,r]^n$ to be an extension of $\bm a$ to dimension $n$. As well, for $i\in [n-1]$, let $\bm e_i \in \{0,1\}^n$ and $\bm e_i^\uparrow \in \{0,1\}^n$ be the $i$th standard basis vectors in dimension $n-1$ and $n$ respectively. By assumption, $F_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$ is $\delta$-close to a linear function $h_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$. Now, for every $x\in[-r-a_i,r-a_i]$ we have
\[F_{\bm a^\uparrow, \bm e_i^\uparrow}(x)=F(a_1,\dots,a_{i-1},a_i+x,a_{i+1},\dots,a_{n-1},c)=F_c(\bm{a}+x\bm{e_i})=(F_c)_{\bm{a,e_i}}(x).\]
Thus, $(F_c)_{\bm{a,e_i}}(x)$ is $\delta$-close to a linear function
%denoted by $(h_c)_{\bm{a,e_i}}(x)$$
on the domain $[-r-a_i,r-a_i]$. Thus, by the inductive hypothesis we can conclude that $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ is $2(n-1)\delta$-close to a multi-linear polynomial $h_c\colon[-r,r]^{n-1}\to\mathbb{R}$. 
 
It remains to show that $F$ is close to a multi-linear polynomial $h$. Let  $h\colon[-r,r]^{n}\to\mathbb{R}$ defined as

 \[h(x_1,\dots,x_n)=\left(\frac{r-x_n}{2r}\right)\underbrace{h_{-r}(x_1,\dots,x_{n-1})}_{multi-linear\ polynomial}+\left(\frac{r+x_n}{2r}\right)\underbrace{h_{r}(x_1,\dots,x_{n-1})}_{multi-linear\ polynomial},\]
The function $h$ is a multi-linear polynomial as both $h_{r}$ and $h_{-r}$ are multi-linear in the formal variables $x_1,\dots,x_{n-1}$. 

Next, we show that $h$ and $F$ are point-wise close on the domain $[-r,r]^n$. Fix $\bm{a}\in [-r,r]^{n-1}$ and let $\bm{a^{\uparrow}}=(a_1,\dots,a_{n-1},0)$, the restriction of $h$ on the line segment $L_{\bm{a^{\uparrow},e_n}}\cap [-r,r]^n$ defined as  $h_{\bm{a^{\uparrow},e_n}}(t)=h(a_1,\dots,a_{n-1},t)$ as a function of the  formal variable $t$ is a univariate linear function as $h_{r}(\bm a)$ and $h_{-r}(\bm a)$ are fixed.
Let $\tilde{h}_{\bm{a^{\uparrow},e_n}}\colon[-r,r]\to\R$ be the a linear fucntion defined by the two end points $\tilde{h}_{\bm{a^{\uparrow},e_n}}(-r)=F_{\bm {a^{\uparrow},e_n}}(-r)$ and  $\tilde{h}_{\bm{a^{\uparrow},e_n}}(r)=F_{\bm {a^{\uparrow},e_n}}(r)$. 
By the assumption $F_{\bm {a^{\uparrow},e_n}}\colon[-r,r]\to\R$ is point-wise $\delta$-close to a linear function.  Therefore it is $2\delta$-close to the linear function $\tilde{h}_{\bm{a^{\uparrow},e_n}}$.
By the induction hypothesis 
\[|h_{r}(\bm a)-\tilde{h}_{\bm{a^{\uparrow},e_n}}(r)|=|h_{r}(\bm a)-F(a_1,\dots,a_{n-1},r)|\leq 2(n-1)\delta\] and \[|h_{-r}(\bm a)-\tilde{h}_{\bm{a^{\uparrow},e_n}}(-r)|=|h_{-r}(\bm a)-F(a_1,\dots,a_{n-1},-r)|\leq 2(n-1)\delta.\]

Therefore $\tilde{h}_{\bm{a^{\uparrow},e_n}}\colon[-r,r]\to\R$ and ${h}_{\bm{a^{\uparrow},e_n}}\colon[-r,r]\to\R$
are $2(n-1)\delta$-point-wise close. 
 
For every $\bm a\in [-r,r]^n$:
\[|h(a)-F(a)|=|h_{(a_1,\dots,a_{n-1}),\bm{e_n}}(a_n)-\tilde{h}_{(a_1,\dots,a_{n-1}),\bm{e_n}}(a_n)|+|\tilde{h}_{(a_1,\dots,a_{n-1}),\bm{e_n}}(a_n)-F(a)|\leq 2(n-1)\delta+2\delta=2n\delta.\]


 \end{proof}


Using the idea from \cite{Kominek89} we prove that $f$ is close to global linear function with blowing up of $n$ in the error. 

\begin{lem}{(Stability version of the Local to Global for degree $1$-functions)}\label{lem:local_to_global}
Let $r \in \mathbb{R}^+$ and $F\colon [-r,r]^n\to\mathbb{R}$. If for every line $L$, the restriction of $F$ on the line segment $L\cap [-r,r]^n$ is point-wise $\delta$-close to a univariate  linear function, then $F\colon [-r,r]^n\to\mathbb{R}$ is point-wise $8n\delta$-close on the hypercube $[-r,r]^n$ to  a linear function $h\colon \R^n\to\mathbb{R}$. 
\end{lem}

\begin{proof}
Let $f^0\colon[r,r]^n\to\R$ defined as 
\[f^0(\bm x)=f(\bm x)-f(\bm 0).\]
Note that any line restriction of $f^0$ is close to a linear function. 
We will show that there exists a global linear function $h^0\colon[-r,r]^n\to\R$ such that $h^0$ and $f^0$ are point-wise close in the cube. Then we define $h(\bm x)=h^0(\bm x)+f(\bm 0)$. 
For every $i\in\{1,\dots,n\}$  define $f_i\colon[-r,r]\to\R$ as 
\[f_i(x)=f^0(x\bm{e_i}).\]
By the assumption there exists a linear function $h_i\colon[-r,r]^n\to \R$ such that for every $x\in [-r,r]$
\[|h_i(x)-f_i(x)|\leq \varepsilon.\]
Let 
\[h^0(\bm x)=\sum_{i=1}^n h_i(x_i).\]
By definition $h^0$ is linear. 
And for every $\bm x\in [-r,r]^n$ 
\[\left|h^0(\bm x)-f^0(\bm x)\right|\leq \underbrace{\left|\sum_{i=1}^n h_i(x_i)-\sum_{i=1}^n f_i(x_i)\right|}_{\leq n\varepsilon}+\underbrace{\left|\sum_i^n f_i(x_i)-f^0(\bm x)\right|}_{=A}\leq 8n\varepsilon.\]
To show that $A\leq 7n\varepsilon$ we 
use an hybrid sum and rewrite it as:
\[A=\left|\sum_{i=1}^n f^0(x_i\bm{e_i})-f^0\left(\sum_{i=1}^n x_i\bm{e_i}\right)\right|=\left|\sum_{j=2}^n\left(f^0(x_j\bm{e_j})-f^0\left(\sum_{i=1}^j x_i\bm{e_i}\right)+f^0\left(\sum_{i=1}^{j-1}x_i\bm{e_i}\right)\right)\right|\leq 7n\varepsilon.\]
The last inequality holds since any line restriction $f^0$ is point-wise close to some linear function intersecting the origin. Therefore $f^0$ is $7\varepsilon$-additive, i.e, for every two points $\bm{x,y,x+y}\in[-r,r]^n$ 
\[|f^0(x+y)-f^0(x)-f^0(y)|\leq 7\varepsilon.\]



\end{proof}



==> tolerant_alterantive.tex <==
\section{Testing Polynomials with Noise - Alternative Definition}

Given input function $f: \R^n \to \R$, we want to distinguish between following two cases with probability $2/3$:
\begin{itemize}
\item
(YES case) There exists a degree-$d$ polynomial $h: \R^n \to \R$ such that for all $\bm{p} \in \R^n$:
\[
|f(\bm{p})-h(\bm{p})| < \delta;
\]
\item
(NO case) For any degree-$d$ polynomial $h: \R^n \to \R$:
\[
\Pr_{\bm{p} \sim \cN(0,I)}[|f(\bm{p})-h(\bm{p})|>2\delta] > \eps.
\]
\end{itemize}



\subsection{Degree-$1$ Univariate Polynomials}

Let $0<a\in \R$ large enough constant (depends on $\varepsilon$) such that 
\[\Pr_{x\sim\cN(0,1)}[x\not\in[-a,a]]\leq \frac{\varepsilon}{2}.\]


\begin{algorithm}[t!]
\caption{Degree-$1$ Univariate Tester}\label{alg:degree_1_univariate}
\Procedure{\emph{\Call{ApproximateLineTester}{$f$}}}{
  \Given {Query access to $f\colon \mathbb{R} \rightarrow \mathbb{R}$, sampling access to the Gaussian distribution $\mathcal{N}(0, 1)$.}
  $\tilde{h}\colon[-a,a]\to\R :=$ be the interpolation of the line passes through the points $(-a,f(-a)),(a,f(a))$\;
  \For{$N := O(\varepsilon^{-1})$ times}{
      Sample $x \sim \mathcal \cN(0,1)$\;
      \If{$x\in[-a,a]$}
      {\textbf{Reject} if $|f(x)-\tilde{h}(x)|\geq 2\delta$\;}
    }
    \textbf{Accept}.
  }  
\end{algorithm}


\begin{thm}{(Univariate degree-$1$ tester with noise)}\label{thm:univariate_degree1_with_noise}

There exists a one-sided error $O\left(\frac{1}{\varepsilon}\right)$-query tester for degree-$1$ functions $f\colon\R\to\R$ over the standard Normal distribution, in the presence of bounded noise. 


\end{thm}

\begin{proof}

Our tester is given in Algorithm \ref{alg:low_degree_main_algorithm}, which defines a degree-$1$ polynomial $\tilde{h}$ on the  range $[-a,a]$ where most of the samples mass is. 
$\tilde{h}$ take the line that passes between the two endpoints $(-a,f(-a))$ and $(a,f(a))$. 
The slop of $\tilde{h}$ is $\frac{f(a)-f(-a)}{2a}$,
and its  y-intercept  is 
$\frac{f(-a)+f(a)}{2}$.

%Therefore $\tilde{h}(x)=\frac{f(a)-f(-a)}{2a}x+\frac{f(-a)+f(a)}{2}$. 
\paragraph{Soundness:}
 In the NO case, $f$ is $\varepsilon$ far from every line and particularly $f$ is far from $\tilde{h}$, the points outside $[-a,a]$ are samples with probability at most $\frac{\varepsilon}{2}$ and therefore, with probability $\frac{\varepsilon}{2}$ points in $[-a,a]$ are far from $\tilde{h}$. Choosing $N$ to be large enough, one of these witnesses will be caught by Algorithm \ref{alg:degree_1_univariate}, with high probability, in this case the tester rejects.
 \paragraph{Completeness:}
We will show that for the YES case $\tilde{h}$ is $2\delta$ close to $f$ for every point in $[-a,a]$ and therefore Algorithm \ref{alg:degree_1_univariate} never reject, thus, we have a perfect completeness.  


\begin{claim}
 Let $f\colon\R\to\R$ be a $\delta$-noisy version of a degree-$1$ univariate polynomial $h\colon\R\to\R$. i.e, For all $x\in \R$, $|f(x)-h(x)|\leq \delta$.
 And Let $\tilde{h}\colon[-a,a]\to\R$ be defined as 
 \[\tilde{h}=\frac{f(a)-f(-a)}{2a}x+\frac{f(-a)+f(a)}{2}.\]
 Then for every $x\in[-a,a]$, $|f(x)-\tilde{h}(x)|\leq 2\delta.$ 
\end{claim}
 
 \begin{proof}
 Let $h(x)=mx+b$ for some $m,b\in\R$. 
 Then $f(-a)=h(-a)+\delta_{-a}=m(-a)+b+\delta_{-a}$ and  $f(a)=ma+b+\delta_a$ for some $\delta_{-a},\delta_a\in [-\delta,\delta]$. 
 Now, we can rewrite 
 \[\tilde{h}(x)=\frac{(ma+b+\delta_a)-(m(-a)+b+\delta_{-a})}{2a}x+\frac{(m(-a)+b+\delta_{-a})+(ma+b+\delta_a)}{2}.\]
 \[\tilde{h}(x)=mx+\frac{\delta_a-\delta_{-a}}{2a}x+b+\frac{\delta_{-a}+\delta_a}{2}=mx+b+\delta_{-a}\frac{a-x}{2a}+\delta_a\left(1-\frac{a-x}{2a}\right).\]
 
 For every $x\in [-a,a]$
 \[|f(x)-\tilde{h}(x)|\leq |f(x)-h(x)|+|h(x)-\tilde{h}(x)|\leq \delta+\left|\delta_{-a}\frac{a-x}{2a}+\delta_a\left(1-\frac{a-x}{2a}\right)\right|\leq 2\delta.\]
 Last inequality is since $-a\leq x\leq a$ we have $0\leq\frac{a-x}{2a}\leq 1$ and both $|\delta_{-a}|$ and $|\delta_a|$ are at most $\delta$.
 \end{proof}
 
 \end{proof}
 
 \subsection{Plan for Degree-$1$ multivariate polynomials}
 
 \paragraph{Local characterization}
 Sample $\bm{p,q}\sim\cN(0,I)$. 
 Reject if $f(\bm{p})$ is $\delta$-far from the line defined by 2 endpoints of the line $L_{\bm{p,q}}$ intersect a reasonable cube (of large enough constant side length) (or a ball).  


Define $g_{\bm{q}}(\bm{p})=\tilde{h}_{\bm{p,q}}(\bm{p})$.
And $g(\bm{p})=Median_{\bm{q}}[g_{\bm{q}}(\bm{p})]$

Show that $g$ on every line is $\delta$-close to degree-$1$ unvariate polinomial. 

Show local to global theorem for the noisy version --- use discretization to find the best one? 

Choose $O\left(\frac{1}{\varepsilon}\right)$ random points $\bm{p}\sim\cN(0,I)$ and reject if they are $2\delta$-far from QUERY-$g(\bm{p})$.

Where QUERY-$g(\bm{p})$ take the Madian of $g_{\bm{q}}(\bm{p})$ out of enough sampled $\bm{q}$.










\subsection{Local to Global with Noise}

\begin{lem}{(Local to Global)}\label{lem:local_to_global}
Let $r \in \mathbb{R}^+$ and $F\colon [-r,r]^n\to\mathbb{R}$. If for every $\bm{a}\in [-r,r]^n,i\in [n]$. The restriction of $F$ on the line segment $L_{\bm{a},\bm{e_i}}\cap [-r,r]^n$ --- the function $F_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$ is point-wise $\delta$-close to a univariate  degree-$d$ polynomial $h_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$, then $F\colon [-r,r]^n\to\mathbb{R}$ is point-wise close to  a multivariate polynomial $h\colon [-r,r]^n\to\mathbb{R}$ which is of degree at most $nd$. 
\end{lem}
\begin{proof}

We show that $F$ is close to a bounded degree ($nd$) polynomial  by induction on the dimension $n$. For the base case when $n=1$, we have that $F=F_{(0,1)}$ and therefore close to a degree-$d$ polynomial by assumption. 

Now, assume the statement is true for dimension $n-1$. 
Let $c\in[-r,r]$ and define $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ as
\[F_c(a_1,\dots,a_{n-1}):=F(a_1,\dots,a_{n-1},c).\]
We will argue that $F_c$ is close to a degree-$(n-1)d$ polynomial $h_c$. 
Fix some $\bm{a}\in[-r,r]^{n-1}$ and define $\bm a^\uparrow=(a_1,\dots,a_{n-1},c) \in [-r,r]^n$ to be an extension of $\bm a$ to dimension $n$. As well, for $i\in [n-1]$, let $\bm e_i \in \{0,1\}^n$ and $\bm e_i^\uparrow \in \{0,1\}^n$ be the $i$th standard basis vectors in dimension $n-1$ and $n$ respectively. By assumption, $F_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$ is close to a degree-$d$ polynomial $h_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$. Now, for every $x\in[-r-a_i,r-a_i]$ we have
\[F_{\bm a^\uparrow, \bm e_i^\uparrow}(x)=F(a_1,\dots,a_{i-1},a_i+x,a_{i+1},\dots,a_{n-1},c)=F_c(\bm{a}+x\bm{e_i})=(F_c)_{\bm{a,e_i}}(x).\]
Thus, $(F_c)_{\bm{a,e_i}}(x)$ is close to a degree-$d$ polynomial 
%denoted by $(h_c)_{\bm{a,e_i}}(x)$$
on the domain $[-r-a_i,r-a_i]$. Thus, by the inductive hypothesis we can conclude that $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ is close to a degree-$(n-1)d$ multivariate polynomial $h_c\colon[-r,r]^{n-1}\to\mathbb{R}$. 
 
It remains to show that $F$ is close to a degree-$nd$ polynomial $h$. Let $c_0,c_1,\dots, c_d\in[-r,r]$ be any $d+1$ distinct values. Using these $d+1$ points, for every $i\in\{0,\dots,d\}$ we define the degree-$d$ polynomial $\delta_{c_i}$ defined uniquely by its evaluation on these $d+1$ points, so that \[\delta_{c_i}(c_j)=\begin{cases}1 & i=j,\\0 &i\neq j.\end{cases}\] 
% Since any degree-$d$ polynomial is defined uniquely by $d+1$ points, for $t \neq c_j$ for all $j$, $\delta_{c_i}(t)$ is well-defined. 
 Using $\delta_{c_i}$, we will show that $h\colon[-r,r]^{n}\to\mathbb{R}$ can be written as a polynomial of degree $nd$.
% \[F(x_1,\dots,x_n)=\sum_{i=0}^{d}\underbrace{\delta_{c_i}(x_n)}_{degree- d}\underbrace{f_{c_i}(x_1,\dots,x_{n-1})}_{degree-(n-1)d}.\]






Define
 \[h(x_1,\dots,x_n)\equiv\sum_{i=0}^{d}\underbrace{\delta_{c_i}(x_n)}_{degree- d}\underbrace{h_{c_i}(x_1,\dots,x_{n-1})}_{degree-(n-1)d},\]
$h$ is degree $nd$ as it defined. It left to show that $h$ and $F$ are point-wise close on the domain $[-r,r]^n$. 

We claim that for every $\bm{a}\in [-r,r]^{n-1}$ and formal variable $t$,
$h_{\bm a}(t)=h(a_1,\dots,a_{n-1},t)$ is degree $d$ as its defined.
Moreover, it close to $F_{(\bm a,0),\bm{e_n}}$ on the points $t=c_0,\dots, c_d$, while by the assumption $F_{(\bm a,0),\bm{e_n}}$ is close to some univariate degree-$d$ function $\tilde{h}$, therefore for every $i\in\{0,\dots,d\}$ we have 
\[|h_{\bm a}(c_i)-\tilde{h}(c_i)|\leq 2\delta.\]

We have to show that this imply that for every $x$ in the cube $|h_{\bm a}(x)-\tilde{h}(x)|\leq 2\delta.$
\enote{Here I stuck with the proof}.\vnote{Noah, and I discussed this, and were inconclusive if this is true. A line of thought: Consider the zeroes of $h_{\bm{a}}(x)-\tilde{h}(x)$. They have to be countable, because if the measure of zeroes of an analytic function $f(=h_{\bm{a}}-\tilde{h})$ is non-zero, then $f\equiv 0$. An example is $h_{\bm{a}}(x)=\tilde{h}(x)+\delta\sin{\pi  x}$. Here $f(x)=0,\forall x\in\mathbb{Z},f\not\equiv 0$, and $|f|\leq\delta$. If the set of zeroes were finite, then consider the largest zero $x_0$. For all $x>x_0,|f(x)|>0$, and $f(x)$ doesn't change sign}
\end{proof}

\paragraph{Linearity Testing (degree-$1$ polynomials)}

\begin{lem}{(Local to Global)}\label{lem:local_to_global}
Let $r \in \mathbb{R}^+$ and $F\colon [-r,r]^n\to\mathbb{R}$. If for every $\bm{a}\in [-r,r]^n,i\in [n]$. The restriction of $F$ on the line segment $L_{\bm{a},\bm{e_i}}\cap [-r,r]^n$ --- the function $F_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$ is point-wise $\delta$-close to a univariate  linear function $h_{\bm{a},\bm{e_i}}:[-r-a_i,r-a_i]\to\mathbb{R}$, then $F\colon [-r,r]^n\to\mathbb{R}$ is point-wise $2n\delta$-close to  a multi-linear polynomial $h\colon [-r,r]^n\to\mathbb{R}$. 
\end{lem}
\begin{proof}

We show that $F$ is $2n\delta$-close to a multi-linear polynomial by induction on the dimension $n$. For the base case when $n=1$, we have that $F=F_{(0,1)}$ and therefore is $\delta$-close to a linear function by assumption. 

Now, assume the statement is true for dimension $n-1$. 
Let $c\in[-r,r]$ and define $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ as
\[F_c(a_1,\dots,a_{n-1}):=F(a_1,\dots,a_{n-1},c).\]
We will argue that $F_c$ is close to a multi-linear function $h_c$. 
Fix some $\bm{a}\in[-r,r]^{n-1}$ and define $\bm a^\uparrow=(a_1,\dots,a_{n-1},c) \in [-r,r]^n$ to be an extension of $\bm a$ to dimension $n$. As well, for $i\in [n-1]$, let $\bm e_i \in \{0,1\}^n$ and $\bm e_i^\uparrow \in \{0,1\}^n$ be the $i$th standard basis vectors in dimension $n-1$ and $n$ respectively. By assumption, $F_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$ is $\delta$-close to a linear function $h_{\bm a^\uparrow, \bm e_i^\uparrow}\colon[-r-a_i,r-a_i]\to\mathbb{R}$. Now, for every $x\in[-r-a_i,r-a_i]$ we have
\[F_{\bm a^\uparrow, \bm e_i^\uparrow}(x)=F(a_1,\dots,a_{i-1},a_i+x,a_{i+1},\dots,a_{n-1},c)=F_c(\bm{a}+x\bm{e_i})=(F_c)_{\bm{a,e_i}}(x).\]
Thus, $(F_c)_{\bm{a,e_i}}(x)$ is $\delta$-close to a linear function
%denoted by $(h_c)_{\bm{a,e_i}}(x)$$
on the domain $[-r-a_i,r-a_i]$. Thus, by the inductive hypothesis we can conclude that $F_c\colon[-r,r]^{n-1}\to\mathbb{R}$ is $2(n-1)\delta$-close to a multi-linear polynomial $h_c\colon[-r,r]^{n-1}\to\mathbb{R}$. 
 
It remains to show that $F$ is close to a multi-linear polynomial $h$. Let  $h\colon[-r,r]^{n}\to\mathbb{R}$ defined as

 \[h(x_1,\dots,x_n)=\left(\frac{r-x_n}{2r}\right)\underbrace{h_{-r}(x_1,\dots,x_{n-1})}_{multi-linear\ polynomial}+\left(\frac{r+x_n}{2r}\right)\underbrace{h_{r}(x_1,\dots,x_{n-1})}_{multi-linear\ polynomial},\]
The function $h$ is a multi-linear polynomial as both $h_{r}$ and $h_{-r}$ are multi-linear in the formal variables $x_1,\dots,x_{n-1}$. 

Next, we show that $h$ and $F$ are point-wise close on the domain $[-r,r]^n$. Fix $\bm{a}\in [-r,r]^{n-1}$ and let $\bm{a^{\uparrow}}=(a_1,\dots,a_{n-1},0)$, the restriction of $h$ on the line segment $L_{\bm{a^{\uparrow},e_n}}\cap [-r,r]^n$ defined as  $h_{\bm{a^{\uparrow},e_n}}(t)=h(a_1,\dots,a_{n-1},t)$ as a function of the  formal variable $t$ is a univariate linear function as $h_{r}(\bm a)$ and $h_{-r}(\bm a)$ are fixed.
Let $\tilde{h}_{\bm{a^{\uparrow},e_n}}\colon[-r,r]\to\R$ be the a linear fucntion defined by the two end points $\tilde{h}_{\bm{a^{\uparrow},e_n}}(-r)=F_{\bm {a^{\uparrow},e_n}}(-r)$ and  $\tilde{h}_{\bm{a^{\uparrow},e_n}}(r)=F_{\bm {a^{\uparrow},e_n}}(r)$. 
By the assumption $F_{\bm {a^{\uparrow},e_n}}\colon[-r,r]\to\R$ is point-wise $\delta$-close to a linear function.  Therefore it is $2\delta$-close to the linear function $\tilde{h}_{\bm{a^{\uparrow},e_n}}$.
By the induction hypothesis 
\[|h_{r}(\bm a)-\tilde{h}_{\bm{a^{\uparrow},e_n}}(r)|=|h_{r}(\bm a)-F(a_1,\dots,a_{n-1},r)|\leq 2(n-1)\delta\] and \[|h_{-r}(\bm a)-\tilde{h}_{\bm{a^{\uparrow},e_n}}(-r)|=|h_{-r}(\bm a)-F(a_1,\dots,a_{n-1},-r)|\leq 2(n-1)\delta.\]

Therefore $\tilde{h}_{\bm{a^{\uparrow},e_n}}\colon[-r,r]\to\R$ and ${h}_{\bm{a^{\uparrow},e_n}}\colon[-r,r]\to\R$
are $2(n-1)\delta$-point-wise close. 
 
For every $\bm a\in [-r,r]^n$:
\[|h(a)-F(a)|=|h_{(a_1,\dots,a_{n-1}),\bm{e_n}}(a_n)-\tilde{h}_{(a_1,\dots,a_{n-1}),\bm{e_n}}(a_n)|+|\tilde{h}_{(a_1,\dots,a_{n-1}),\bm{e_n}}(a_n)-F(a)|\leq 2(n-1)\delta+2\delta=2n\delta.\]


 \end{proof}


Using the idea from \cite{Kominek89} we prove that $f$ is close to global linear function with blowing up of $n$ in the error. 

\begin{lem}{(Stability version of the Local to Global for degree $1$-functions)}\label{lem:local_to_global}
Let $r \in \mathbb{R}^+$ and $F\colon [-r,r]^n\to\mathbb{R}$. If for every line $L$, the restriction of $F$ on the line segment $L\cap [-r,r]^n$ is point-wise $\delta$-close to a univariate  linear function, then $F\colon [-r,r]^n\to\mathbb{R}$ is point-wise $8n\delta$-close on the hypercube $[-r,r]^n$ to  a linear function $h\colon \R^n\to\mathbb{R}$. 
\end{lem}

\begin{proof}
Let $f^0\colon[r,r]^n\to\R$ defined as 
\[f^0(\bm x)=f(\bm x)-f(\bm 0).\]
Note that any line restriction of $f^0$ is close to a linear function. 
We will show that there exists a global linear function $h^0\colon[-r,r]^n\to\R$ such that $h^0$ and $f^0$ are point-wise close in the cube. Then we define $h(\bm x)=h^0(\bm x)+f(\bm 0)$. 
For every $i\in\{1,\dots,n\}$  define $f_i\colon[-r,r]\to\R$ as 
\[f_i(x)=f^0(x\bm{e_i}).\]
By the assumption there exists a linear function $h_i\colon[-r,r]^n\to \R$ such that for every $x\in [-r,r]$
\[|h_i(x)-f_i(x)|\leq \varepsilon.\]
Let 
\[h^0(\bm x)=\sum_{i=1}^n h_i(x_i).\]
By definition $h^0$ is linear. 
And for every $\bm x\in [-r,r]^n$ 
\[\left|h^0(\bm x)-f^0(\bm x)\right|\leq \underbrace{\left|\sum_{i=1}^n h_i(x_i)-\sum_{i=1}^n f_i(x_i)\right|}_{\leq n\varepsilon}+\underbrace{\left|\sum_i^n f_i(x_i)-f^0(\bm x)\right|}_{=A}\leq 8n\varepsilon.\]
To show that $A\leq 7n\varepsilon$ we 
use an hybrid sum and rewrite it as:
\[A=\left|\sum_{i=1}^n f^0(x_i\bm{e_i})-f^0\left(\sum_{i=1}^n x_i\bm{e_i}\right)\right|=\left|\sum_{j=2}^n\left(f^0(x_j\bm{e_j})-f^0\left(\sum_{i=1}^j x_i\bm{e_i}\right)+f^0\left(\sum_{i=1}^{j-1}x_i\bm{e_i}\right)\right)\right|\leq 7n\varepsilon.\]
The last inequality holds since any line restriction $f^0$ is point-wise close to some linear function intersecting the origin. Therefore $f^0$ is $7\varepsilon$-additive, i.e, for every two points $\bm{x,y,x+y}\in[-r,r]^n$ 
\[|f^0(x+y)-f^0(x)-f^0(y)|\leq 7\varepsilon.\]



\end{proof}


\section{Testing Additivity with Bounded Noise for the Standard Gaussian }\label{sec:additivity}



Given input function $f: \R^n \to \R$ and $\varepsilon >0.01$ \enote{$\varepsilon$ can be arbitrarily small, and the resulting radius is parameterized by $\varepsilon$},  we want to distinguish between following two cases with probability $2/3$:
\begin{itemize}
\item
(YES case) There exists an additive function $F: \R^n \to \R$ such that for all $\bm{p} \in \R^n$:
\[
|f(\bm{p})-F(\bm{p})| < \alpha;
\]
\item
(NO case) For any additive function  $F: \R^n \to \R$:
\[
\Pr_{\bm{p} \sim \cN(0,I)}[|f(\bm{p})-F(\bm{p})|>20n^2\alpha] > \eps.
\]
\end{itemize}


\subsection{Preliminaries}
The following two are from \cite{Kominek89} and show stability version of local to global lemma.
% \begin{lem}[\cite{Kominek89},Lemma 2.]\label{lem:closeness_to_additivity}
%   If $f\colon(-r,r)^n\to\R$ is $\delta$-additive in $(-r,r)^n$ then there exists an additive function $h\colon\R^n\to\R$ such that for every $\bm x\in (-r,r)^n$ 
%   \[|f(\bm x)-h(\bm x)|\leq 5n\delta.\]
% \end{lem}
\begin{thm}[\cite{Kominek89},Theorem 2.]\label{lem:closeness_to_additivity_on_ball}
Let $f\colon\ball(\bm 0,R)\to \R$, if $f$ is $\delta$-additive in $\ball(\bm 0,R)$ (where $\ball(\bm 0,R)$ is of dimension $n$) then there exists additive function $h\colon\R^n\to\R$ 
that for every $\bm x\in \ball(\bm 0,R)$ 
  \[|f(\bm x)-h(\bm x)|\leq 5n^{1.5}\delta.\]
\end{thm}
Few points
\begin{itemize}
    \item We rely on the exact case additivity tester and a stability theorem for additive functions: 
    \item We changed the tests to test closeness instead of equality
    \item We define $g$ in the small ball as the median value of $g_{\bm{x}}(\bm{p})=f(\bm{p}+\bm{x})-f(\bm{x})$, and then prove that we can query $g$ inside the small ball with high probability and small error. 
    \item We then show that $g$ is $\delta$-additive inside the small ball.
    \item By Lemma 2.2 \enote{maybe better to use Theorem 2.2}  from \cite{Kominek89} we have that there exists additive function $h\colon\R^n\to\R$ that $\delta n$-point-wise close to $g$ on the small ball.
    \item Define the NO case: for every additive function $h'$, $\Pr_{\bm{x}\sim \cN(0,I)}[|f(\bm{x})-h'(\bm{x})|>n^2\delta]\geq \varepsilon$. Thus we will not test points outside the large ball ( that catch most of the mass) 
    \item For points inside the large ball: note that $h$ is additive, therefore $h(\bm{0})=0$, and $ h(\bm{p})=\kappa_{\bm{p}}\cdot h\left(\frac{\bm{p}}{\kappa_{\bm{p}}}\right)$, 
    and we have
    $\left|h\left(\frac{\bm{p}}{\kappa_{\bm{p}}}\right)-g\left(\frac{\bm{p}}{\kappa_{\bm{p}}}\right)\right|\leq \delta n$,
    
    therefore $\left|h(\bm{p})-\kappa_{\bm{p}} g\left(\frac{\bm{p}}{\kappa_{\bm{p}}}\right)\right|\leq \kappa_{\bm{p}}\delta n$. 
    
    \item In the yes case - we note that $g$ is close to both $f$ and $h$- we need to analyze the error blow up when querying points outside the small ball. 
\end{itemize}








Our goal in this section is to design a constant-query  tester for the additivity of a  function $F\colon \mathbb{R}^n \rightarrow \mathbb{R}$ over the standard Gaussian where we have a query access to $f$ which gives the values of $F$ within accuracy of up to $\alpha$.



Note that if the underlying function $F\colon\R^n\to\R$ of $f$ is additive and for every $\bm p\in \R^n$ we have bounded error $|F(\bm p)-f(\bm p)|\leq \alpha$ then $f$ is $\delta$-additive everywhere for $\delta=3\alpha$. i.e., for every $\bm p,\bm q\in \R^n$
\[|f(\bm p+\bm q)-f(\bm p)-f(\bm q)|\leq \delta.\]

\begin{thm}\label{thm:central-gausssian}
  There exists a one-sided error $O\left(\frac{1}{\varepsilon} \log\frac{1}{\varepsilon}\right)$-query tester for testing additivity in the presence of bounded noise over the standard Gaussian.
  % which succeeds with probability at least $1-(\alpha + \sigma)$.
\end{thm}



At a high-level, our tester consists of two steps. First, we test whether $f$ satisfies $\delta$-additivity over a set of samples drawn from the distributions $\cN(\bm 0,I),\cN(\bm 0,\frac{1}{2}I)$. If $f$ passes this test, then we conclude that there must be a $O(\delta)$-additive function $g$, which is a self-corrected version of $f$ on some small ball and is $O(n^{1.5}\delta$)-close to an additive function $h\colon\R^n\to\R$. Second, by testing the value of $f$ on a correlated set of points, we are able to get approximate values of $g$ inside the same small ball with high probability. So, we can simply estimate the distance between $f$ and $g$, and therefore between $f$ and $h$.

For points $\bm p$ outside the ball, we map them to the corresponding point inside the ball, by dividing by an appropriate contraction factor $\kappa_{\bm p}$, defined later. We approximate $h$ on the corresponding point $\bm p/\kappa_{\bm p}$ inside the ball, and using homogeneity of $h$, map $h(\bm p/\kappa_{\bm p})$ back to $h(\bm p)$.

Our tester relies on the fact that it has one-sided error: if the underlying function of $f$ is additive then our test passes with probability $1$. Otherwise, if $f$ is far from any additive function  and the second step passes with high probability, then $f$ and $h$ must be far.

The evaluation of the function $g$ at a point $\bm{p}\in\ball(\bm 0,R)$ is defined as the (weighted) Median value of $g_{\bm{x}}(\bm{p})\triangleq f(\bm{p}-\bm{x}) + f(\bm{x})$ over all $\bm{x} \sim \mathcal{N}(\bm 0,I)$ (where, $g_{\bm{x}}(\bm{p})$ is weighted according to the probability of drawing $\bm{x} \sim \mathcal{N}(\bm 0,I)$). 
%However, there are some significant challenges in generalizing the BLR test to the standard Gaussian, the most obvious of which is that unlike the uniform distribution, every point in the support of the distribution does not have equal probability. In particular, $p-x$ is not distributed as $x \sim \mathcal{N}(0,I)$ for fixed $p \neq 0$. In order to overcome this, we exploit the fact that for additive functions $f$, we have $f(x) = q f(x/q)$ for every rational $q$. 
We first restrict attention to a small ball $\ball(\bm 0,R)$ of radius $R$ centered at the origin. Then, for $\bm p \in \ball(\bm 0,R)$, $\bm p -\bm x$ is approximately distributed as $\bm x$ for small enough $R$. We define $g$ within $\ball(\bm 0,R)$, and then extrapolate to define $g$ on a large ball that contains most of the mass $1-\frac{\varepsilon}{4}$ of $\cN(\bm 0,I)$. That blows up the error by $\sqrt{n}$.

Concretely, we will define $g$ as follows. First, let $R$ be a sufficiently small rational  ($R=1/50$ suffices). For each point $\bm p \in \mathbb{R}^n$, define
\[ k_{\bm p} := \begin{cases} 1 &\text{ if } \|\bm p \|_2 \leq R, \\ \left \lceil \frac{ \|\bm p\|_2 }{R}\right \rceil   &\text{ if } \|\bm p \|_2 > R. \end{cases}\]
Now, define $g\colon\mathbb{R}^n \rightarrow \mathbb{R}$\enote{Maybe define g only inside the ball} as
\[ g(\bm p) := k_{\bm p} \cdot \mathop{\mathsf{Median}}_{\bm x\sim\mathcal{N}(0,I)} \left[  g_{\bm x} \left( \frac{\bm p}{\kappa_{\bm p}} \right)  \right] = k_{\bm p} \cdot \mathop{\mathsf{Median}}_{\bm x\sim\mathcal{N}(0,I)} \left[  f \left( \frac{\bm p}{k_{\bm p}}- \bm x \right) +f \left (\bm x \right)  \right], \]
where ${\mathsf{Median}}_{\mathcal{N}(0,I)}$ is the weighted median of the  value $g_{\bm x}(\bm p/\kappa_{\bm p})$, with $\bm x$ being weighted according to its probability mass under $\bm x \sim \mathcal{N}(0,I)$. Observe that either $\bm p \in \ball(0,R)$, in which case we can approximate $h(\bm p)$ by approximating $g(\bm p)$, or $\bm p\not\in\ball(\bm 0,R)$, wherein approximating $h(\bm p)$ first maps $\bm p$ to a point $\bm p/k_{\bm p}$ in $\ball(\bm 0,R)$. The value of $g$ inside $\ball(\bm 0,R)$ is the median value (according to $\mathcal{N}(\bm 0,I)$) of  $g_{\bm x}(\bm p/\kappa_{\bm p}) = f(\bm p/k_{\bm p} -\bm x) + f(\bm x)$. If $f$ is close to additive, then taking this Median should allow us to approximately correct for the errors in $f$.


\begin{figure}[H]
\center
\begin{tikzpicture}[scale=0.8]
  \draw[fill=green!05] (0,0) circle (2cm);
  \draw[red!56, very thick] (0,0) circle (1cm);

  \draw[black!60, very thick] (0,-3.5)  -- (-0,3.5);
  \draw[black!60, very thick] (-3.5,0)  -- (3.5,0);
  \draw[black!60, thick ,dashed] (1.4,-1.4)  -- (-0,0);

  \node[text width=.5cm] at (0.9 ,1.5) {$\bm p$};
  \node[text width=.5cm] at (0 , 0.4) {$\bm 0$};
  \node[text width=.5cm] at (1.3 , -0.8) {$R$};
    \end{tikzpicture}
  \caption{The Ball in which we know to estimate the value of $h$}
  \label{fig:proj2dPlane}
\end{figure}
\vspace{1em}

\begin{algorithm}[!t]
  \caption{Standard Gaussian Additivity Tester}\label{alg:zero-mean-additivity}
%  \Procedure{\emph{\Call{TestZeroMeanGaussianAdditivity}{$f,\Sigma$}}}{
    \Given{Query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, sampling access to the distribution $\mathcal{N}(0, I)$;}
    \textbf{Reject} if \Call{TestAdditivity}{$f$} returns \textbf{Reject}\;
    \For{$N_{\ref{alg:zero-mean-additivity}} := O(1/\varepsilon)$ times}{
      Sample $\bm p \sim \mathcal{N}(0,I)$\;
      \If{ $\bm p\in \ball(\bm 0, 10\sqrt{n})$}{
      \textbf{Reject} if $|f(\bm p) -$ \Call{Approximate-$g$}{$\bm p,f$}$|>5\delta n^{1.5}\kappa_{\bm p}$  or if \Call{Approximate-$g$}{$\bm p,f$} returns \textbf{Reject}.}
    }
    \textbf{Accept}.
%  }
\end{algorithm}
\begin{algorithm}[!t]
  \caption{Subroutines}\label{alg:subroutines}
  \Procedure{\emph{\Call{TestAdditivity}{$f$}}}{
    \Given{Query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, sampling access to the distribution $\mathcal{N}(0, I)$;}
    \For{$N_{\ref{alg:subroutines}} := O(1)$ times}{
      Sample $\bm x,y,z \sim \cN(\bm 0, I), \bm w \sim \mathcal{N}(0,(1/2)I)$\;
      \textbf{Reject} if $|f(-\bm x)+f(\bm x)|>2\delta$\;
      \textbf{Reject} if $|f(-\bm w)+f(\bm w)|>2\delta$\;
      \textbf{Reject} if $|f(\bm x - \bm y) - \left(f(\bm x) - f(\bm y)\right)|>\delta$\;
      \textbf{Reject} if $|f(\bm x - \bm w) - \left(f(\bm x) - f(\bm w)\right)|>\delta$\;
      \textbf{Reject} if $\left|f\left(\frac{\bm x - \bm y}{2} \right) - \left( f \left(\frac{\bm x -\bm z}{2} \right) + f \left(\frac{\bm z - \bm y}{2} \right)\right)\right|>3\delta$\;
      %Sample $\bm x, \bm y, \bm z \sim \mathcal{N}(0,\frac{1}{2}I)$\;
      %\textbf{Reject} if $|f(-\bm x)+f(\bm x)|>2\delta$\;
      %\textbf{Reject} if $|f(x - y) - f(x) + f(y)|>\delta$\;
      %\textbf{Reject} if $\left|f\left(\frac{x-y}{2} \right) - f \left(\frac{x - z}{2} \right) - f \left(\frac{z - y}{2} \right)\right|>3\delta$\;
    }
    \textbf{Accept}.
  }
  \Procedure{\emph{\Call{Approximate-$g$}{$\bm p, f$}}}{
    \Given{$p \in \mathbb{R}^n$, query access to $f\colon \mathbb{R}^n \rightarrow \mathbb{R}$, sampling access to $\mathcal{N}(0,I)$;}
    $N'_{\ref{alg:subroutines}} := O\left(\log \frac{1}{\varepsilon}\right)$\;
    Sample $\bm x_{1}, \ldots, \bm x_{N'_{\ref{alg:subroutines}}} \sim \mathcal{N}(0,I)$\;
    \textbf{Reject} if there exists $i,j \in [ N'_{\ref{alg:subroutines}}]$ such that $\left|\left(f(\bm p/k_{\bm p} - \bm x_i) + f(\bm x_i)\right) -\left(f(\bm p/k_{\bm p} - \bm x_j) + f(\bm x_j)\right)\right|>6\delta$\;
    \Return $k_{\bm p} \left( f( \bm p/k_{\bm p} - \bm x_1) + f(\bm x_1) \right)$.
  }
\end{algorithm}

% \begin{mdframed}
%   \begin{algorithms}[Mean-Zero Gaussian Additivity Tester]\label{alg:zero-mean-additivity}\mbox{} \vspace{0.2em}
%     \hrule
%     \begin{description}
%     \item[Given:]
%         Query access to $f: \mathbb{R}^n \rightarrow \mathbb{R}$, sample access to the distribution $\mathcal{N}(0, \Sigma)$;
%     %\item[Output:]
%      % \emph{Yes} iff $f$ is $\varepsilon$-close to additive.
%     \item[Operation:]\mbox{}
%       \begin{enumerate}
%       \item {\bf Reject} if \Call{TestAdditivity}{}$(\Sigma)$ returns reject.
%       \item Sample $p_1, \ldots, p_{\frac{1}{\varepsilon - \kappa} \ln\frac{1}{\sigma}} \sim \mathcal{N}(0,\Sigma)$.
%       \item For each $i \in \left[ \frac{1}{\varepsilon - \kappa} \ln\frac{1}{\sigma} \right]$,
%       \begin{enumerate}
%         \item[i.] {\bf Reject} if $f(p_i) \neq$ \emph{Query-}$g(p_i,\Sigma)$ or if \emph{Query-}$g(p_i, \Sigma)$ returns reject.
%       \end{enumerate}
%       \item {\bf Accept}.
%     \end{enumerate}

%     \end{description}
%   \end{algorithms}
% \end{mdframed}

% \begin{mdframed}
%   \begin{subroutine}[TestAdditivity]\label{alg:zero-mean-additivity}\mbox{} \vspace{0.2em}
%     \hrule
%     \begin{description}
%     \item[Given:]
%         Query-Access to $f: \mathbb{R}^n \rightarrow \mathbb{R}$, sample access to the distribution $\mathcal{N}(0, \Sigma)$;
%     %\item[Output:]
%      % \emph{Yes} iff $f$ is $\varepsilon$-close to additive.
%     \item[Operation:]\mbox{}
%       \begin{enumerate}
%       \item Sample $(x_1, y_1, z_1), \ldots, (x_{\frac{1}{\psi} \ln\frac{1}{\alpha}}, y_{\frac{1}{\psi} \ln\frac{1}{\alpha}}, z_{\frac{1}{\psi} \ln\frac{1}{\alpha}}) \sim \mathcal{N}(0,\Sigma)$.
%       \item {\bf Reject} if there exists $i \in [\frac{1}{\psi} \ln\frac{1}{\alpha}]$ such that $f(x_i - y_i) \neq f(x_i) - f(y_i)$.
%       \item {\bf Reject} if there exists  $i \in [\frac{1}{\psi} \ln\frac{1}{\alpha}]$ such that $f(-x_i) \neq -f(x_i)$.
%       \item {\bf Reject} if there exists  $i \in [\frac{1}{\psi} \ln\frac{1}{\alpha}]$ such that $f\left(\frac{x_i-y_i}{2} \right) \neq f \left(\frac{x_i - z_i}{2} \right) + f \left(\frac{z_i - y_i}{2} \right)$.
%       \item {\bf Accept}.
%     \end{enumerate}

%     \end{description}
%   \end{subroutine}
% \end{mdframed}

% \begin{mdframed}
%   \begin{subroutine}[Query-$g$]\label{sub:Query-g}\mbox{} \vspace{0.2em}
%     \hrule
%     \begin{description}
%     \item[Given:]
%         $p \in \mathbb{R}^n$, query-Access to $f: \mathbb{R}^n \rightarrow \mathbb{R}$, sample access to $\mathcal{N}(0, \Sigma)$;
%     %\item[Output:]
%      % \emph{Yes} iff $f$ is $\varepsilon$-close to additive.
%     \item[Operation:]\mbox{}
%       \begin{enumerate}
%       %\item Define
%       % $k_p := \begin{cases} 1 &\mbox{ if } \|p \|_2 \leq 1/r, \\ 2 \left \lceil r \cdot \|p\|_2 \right \rceil   &\mbox{ if } \|p \|_2 > 1/r. \end{cases}$.
%       \item Sample $x_{1}, \ldots, x_{\log(1/\kappa)} \sim \mathcal{N}(0,\Sigma)$.
%       \item {\bf Reject} if there exists $i,j \in [ \log(1/\kappa)]$ such that $f(\frac{1}{k_p} p - x_i) + f(x_i) \neq f(\frac{1}{k_p} p - x_j) + f(x_j)$
%       \item {\bf Return} $k_p \left( f( \frac{1}{k_p} p-x_1) + f(x_1) \right)$
%     \end{enumerate}
%     \end{description}
%   \end{subroutine}
% \end{mdframed}

Our tester is given in Algorithm~\ref{alg:zero-mean-additivity}, which uses subroutines given in Algorithm~\ref{alg:subroutines}.
The \Call{Approximate-$g$}{} subroutine allows us to obtain query access to  values close enough to $g$ with high probability, while the \Call{TestAdditivity}{} subroutine tests the conditions that we require in order to prove that $g$ is $\delta$-additive.

\begin{lem}\label{lem:g-is-additive}
  If \Call{TestAdditivity}{$f$} accepts with probability at least $1/10$, then $g$ is a $30\delta$-additive function inside the small ball $\ball(\bm 0,R)$, and furthermore, for every $\bm p\in\ball(\bm 0,R)$  it holds that 
  \[\Pr_{\bm x \sim \mathcal{N}(\bm 0,I)}[\left|g(\bm p) - \left( f(\bm p - \bm x) + f(\bm x)\right)\right|\geq 6\delta ] < 1/2.\]
\end{lem}

We first prove Theorem~\ref{thm:central-gausssian} assuming that Lemma~\ref{lem:g-is-additive} holds.
\begin{proof}[Proof of Theorem~\ref{thm:central-gausssian}]
  First, observe that if $f$ is a noisy version of an additive function with noise bounded by $\alpha$, then $f$ is a $\delta$-additive function for $\delta=3\alpha$, and then Algorithm~\ref{alg:zero-mean-additivity} always accepts. Indeed, it is immediate that \Call{TestAdditivity}{$f$} always accepts. To see that $f$ also passes the remaining tests, observe that by $\delta$-additivity,  $\left|k_{\bm p} \left( f(\bm p/k_{\bm p} - \bm x) + f(\bm x) \right) - f(\bm p)\right|\leq 2\delta \kappa_{\bm p}$.
  \enote{Is it trivial of need to show in prelims? } Note, that \Call{Approximate-$g$}{$\bm p, f$} never rejects, because we have $\left| \left( f(\bm p/\kappa_{\bm p} - \bm x) + f(\bm x) \right) - f(\bm p)/\kappa_{\bm p}\right|\leq 2\delta$. Then, 
  \begin{align*}
      |f(\bm p/\kappa_{\bm p}-\bm x_i)-f(\bm x_i)-(f(\bm p/\kappa_{\bm p}-\bm x_j)+f(\bm x_j))|\leq \left|\left( f(\bm p/\kappa_{\bm p} - \bm x) + f(\bm x) \right) - f(\bm p)/\kappa_{\bm p}\right|\leq 2\delta
  \end{align*}
  %, where the final inequality holds because $k_p \in \mathbb{Z}$ and by homogeneity over the rationals $f(qx) = qf(x)$ for every $q \in \mathbb{Q}$.

  We now show that if $f$ is $\varepsilon$-far from all $\delta_1 n$-additive functions, then Algorithm~\ref{alg:zero-mean-additivity} rejects with probability at least $2/3$.
  If \Call{TestAdditivity}{$f$} accepts with probability at most $1/3$, we can reject $f$ with probability at least $2/3$.
  Hence, we assume that \Call{TestAdditivity}{$f$} accepts with probability at least $2/3$.
  Then by \autoref{lem:g-is-additive}, the function $g$ is $\delta$-additive. 
  Using Lemma 2 from \cite{Kominek89}, there is an additive function $h\colon\R^n\to\R$,  which is 
  $5\delta n$-close to $g$ on the small ball, and hence $f$ is $\varepsilon$-far from $h$.
%  Note that we can decrease the acceptance probability to $1/3$ by running Algorithm~\ref{alg:zero-mean-additivity} a constant number of times and then accept if and only if all the runs accept.
  Now, we want to bound the probability that Step~2 of Algorithm~\ref{alg:zero-mean-additivity} passes.
%  It remains to show that if Algorithm~\ref{alg:zero-mean-additivity} accepts with probability $1-(\alpha+ \sigma)$, then the functions $f$ and $g$ are $\varepsilon$-close.
%  Note that by Lemma~\ref{lem:g-is-additive}, we can conclude that $f$ is $\varepsilon$-close to an additive function with error probability at most $\alpha$. Therefore, we want to bound the probability that Step 3 of Algorithm~\ref{alg:zero-mean-additivity} passes, but $f$ and $g$ are $\varepsilon$-far.

  First, we bound the probability that \Call{Approximate-$g$}{$\bm p, f$} fails to recover the value of $g(\bm p)$ within an error of $4\delta$. That is, we bound the probability that $\left|\left(f(\bm p/k_{\bm p} -\bm x_i) + f(\bm x_i)\right)-\left( f(\bm p/k_{\bm p} -\bm x_j) + f(\bm x_j)\right)\right|\leq 2\delta$, for all $i,j \in \left[ N'_{\ref{alg:subroutines}} \right]$, but $\left|g(\bm p) -\left( k_{\bm p} \left( f(\bm p/k_{\bm p} - \bm x_i) + f(\bm x_i) \right)\right)\right|>4\delta$.
  By Lemma~\ref{lem:g-is-additive}, the probability that we draw $N'_{\ref{alg:subroutines}}$ points which satisfy this is at most $2^{-N'_{\ref{alg:subroutines}}} \leq \varepsilon /4$, by choosing the hidden constant in $N'_{\ref{alg:subroutines}}$ to be large enough. Therefore, the probability that we correctly recover a value close enough to $g(\bm p)$ is at least $1-\varepsilon/4$.

  Now that we have established that we can obtain query access to $g$ with high probability, it remains to show that we can test whether $f$ and $h$ are close.
  Indeed, the probability that Step~2 of Algorithm~\ref{alg:zero-mean-additivity} fails to reject is at most
  \begin{align*}
    & {\left( \Pr_{\bm p \sim \mathcal{N}(0,I)} \left[ \left|f(\bm p)- g(\bm p)\right|\leq 2\delta n \vee \text{\Call{Approximate-$g$}{$\bm p, f$} fails to correctly recover $g(\bm p)$} \right]  \right)}^{N_{\ref{alg:zero-mean-additivity}}} \\
    \leq & {\left( 1- \Pr_{\bm p \sim \mathcal{N}(0,I)} [\left|f(\bm p)- g(\bm p)\right|>2\delta n] + \Pr_{\bm p \sim \mathcal{N}(0,I)} \left[ \text{\Call{Approximate-$g$}{$\bm p, f$} fails to correctly recover $g(\bm p)$} \right]  \right)}^{N_{\ref{alg:zero-mean-additivity}}} \\
    <& {\left(1- \frac{\varepsilon}{4} \right)}^{N_{\ref{alg:zero-mean-additivity}}} < \frac{1}{3},
  \end{align*}
  by choosing the hidden constant in $N_{\ref{alg:zero-mean-additivity}}$ to be large enough.
  Therefore, Algorithm~\ref{alg:zero-mean-additivity} rejects with probability at least $2/3$.
%  This completes the proof of Theorem~\ref{thm:central-gausssian}.
\end{proof}

It remains to prove Lemma~\ref{lem:g-is-additive} showing that if  Algorithm~\ref{alg:zero-mean-additivity} succeeds, then $g$ is an additive function with high probability.

\enote{Need to add: We don't test points outside large ball (of radius $\sqrt(n)$?)  the mass there is at most $\frac{\varepsilon}{4}$ and then in the no case we left with at least $\frac{3\varepsilon}{4}$ probability to catch a witness. }

\enote{Need to analyze how much we loose in the error when testing points that are outside the small ball.}

\subsubsection{$100\delta$-Additivity of the Function $g$}
First, we record the basic, but useful observation that if the \Call{TestAdditivity}{} subroutine passes then each of its tests hold with high probability over $\mathcal{N}(\bm 0,I)$ and $\cN(\bm 0,(1/2)I)$.

\begin{lem}\label{lem:f-additive-whp}
  If \Call{TestAdditivity}{$f$} accepts with probability at least $1/10$, then 
  \begin{align} 
    \Pr_{\bm x \sim \mathcal{N}(\bm 0, I)}[\left|f(-\bm x) + f(\bm x)\right|\leq 2\delta] \geq \frac{99}{100}, \label{eq:lem3-1} \\
  \Pr_{\bm x \sim \mathcal{N}(\bm 0, (1/2)I)}[\left|f(-\bm x) + f(\bm x)\right|\leq 2\delta] \geq \frac{99}{100}, \label{eq:lem3-2} \\
  \Pr_{\bm x,y \sim \mathcal{N}(\bm 0,I)} \left [\left|f(\bm x - \bm y) - f(\bm x) + f(\bm y)\right|\leq \delta \right] \geq \frac{99}{100}, \label{eq:lem3-3} \\
  \Pr_{\substack{\bm x \sim \mathcal{N}(\bm 0,I) \\ \bm y \sim \cN( \bm{0}, (1/2)I)}} \left [\left|f(\bm x - \bm y) - f(\bm x) + f(\bm y)\right|\leq \delta \right] \geq \frac{99}{100}, \label{eq:lem3-4} \\
   \Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(\bm 0,I)} \left [\left|f\left(\frac{\bm x - \bm y}{2} \right) - f \left(\frac{\bm x - \bm z}{2} \right) - f \left(\frac{\bm z - \bm y}{2} \right)\right|\leq 3\delta \right] \geq \frac{99}{100}.  \label{eq:lem3-5}%\\
%   \Pr_{\bm x,\bm y \sim \mathcal{N}(0,\frac{1}{2}I)} \left [\left|f(\bm x - \bm y) - f(\bm x) + f(\bm y)\right|\leq \delta \right] \geq \frac{99}{100}, \label{eq:lem3-4} \\
%   \Pr_{\bm x \sim \mathcal{N}(0,\frac{1}{2}I)}[\left|f(-\bm x) + f(\bm x)\right|\leq 2\delta] \geq \frac{99}{100}, \label{eq:lem3-5} \\
%   \Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(0,\frac{1}{2}I)} \left [\left|f\left(\frac{\bm x - \bm y}{2} \right) - f \left(\frac{\bm x - \bm z}{2} \right) - f \left(\frac{\bm z - \bm y}{2} \right)\right|\leq 3\delta \right] \geq \frac{99}{100}.  \label{eq:lem3-6} \\
%   \Pr_{\bm x\sim \mathcal{N}(0,I),\bm y \sim \mathcal{N}(\bm 0,(1/2)I)} \left [\left|f(\bm x - \bm y) - f(\bm x) + f(\bm y)\right|\leq \delta \right] \geq \frac{99}{100}, \label{eq:lem3-additivity_gaussian_vs_scaled} \\
%   \Pr_{\bm x \sim \mathcal{N}(0,\frac{3}{8}I)}[\left|f(-\bm x) + f\bm (x)\right|\leq 2\delta] \geq \frac{99}{100}, \label{eq:lem3-8} \\
%   \Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(0,\frac{3}{8}I)} \left [\left|f\left(\frac{\bm x - \bm y}{2} \right) - f \left(\frac{\bm x - \bm z}{2} \right) - f \left(\frac{\bm z - \bm y}{2} \right)\right|\leq 3\delta \right] \geq \frac{99}{100}.  \label{eq:lem3-9}
  \end{align}
\end{lem}
\begin{proof}
  Suppose for contradiction that at least one of~\eqref{eq:lem3-1},~\eqref{eq:lem3-2}, ~\eqref{eq:lem3-3},~\eqref{eq:lem3-4} and ~\eqref{eq:lem3-5}%,~\eqref{eq:lem3-6},~\eqref{eq:lem3-7},~\eqref{eq:lem3-8}, and~\eqref{eq:lem3-9} 
  does not hold.
  We here assume that~\eqref{eq:lem3-1} does not hold as other cases are similar.

  We accept only when all the sampled pairs $(\bm x,\bm y)$ satisfy $|f(\bm x + 
  \bm y) -f(\bm x) - f(\bm y)|\leq \delta$.
  By setting the hidden constant in $N_{\ref{alg:subroutines}}$ to be large enough, this happens with probability at most
  \[ {\left(1- \Pr_{\bm x,\bm y \sim \mathcal{N}(0,I)} [|f(\bm x + \bm y) - f(\bm x) - f(\bm y)|>\delta] \right)}^{N_{\ref{alg:subroutines}}} < {\left( \frac{99}{100}\right)}^{N_{\ref{alg:subroutines}}} < \frac{1}{10}, \]
  which is a contradiction.
  % By similar arguments we have the same bound of $\alpha/3$ for
  % ,~\eqref{eq:lem3-2} and~\eqref{eq:lem3-3} each hold with probability at least $1-\alpha/3$ as well. Therefore, by a union bound, the probability that all three hold simultaneously is at least $1-\alpha$.
\end{proof}

In order to argue that $g$ is $100\delta$-additive, we will first argue that $g$ is $100\delta$-additive on points within the tiny ball $
\ball(0,R)$. To do so, we will crucially use the fact that $\bm p - \bm x$ is distributed approximately as $\bm x \sim \mathcal{N}(0,I)$, if $\|\bm p\|_2$ is small.
%Therefore, we set the value of $r$ to be $50$.
By \autoref{lem:usefulDTVBound}, we have a bound on the total variation distance between $\bm x$ and $\bm x + \bm p$.
\begin{claim}\label{clm:tvd-bound-on-ball}
  Let $\bm p \in \mathbb{R}^n$ satisfying $\|\bm p\|_2 \leq kR$, for some $k \in \mathbb{Z}^{>0}$.
  Then $\dtv(\mathcal{N}(\bm 0,I), \mathcal{N}(\bm p, I)) \leq k /100$.
\end{claim}
\begin{proof}
	Since, $\|\bm p\|_2 \leq kR$, by \autoref{lem:usefulDTVBound}, 
	we claim $\dtv(\cN(\bm 0,I),\cN(\bm p,I))\leq kR/2\leq k/100$, since $R\leq 1/50$.
\end{proof}

After arguing that $g$ is $100\delta$-additive in $\ball(\bm 0,R)$, it will follow using Lemma 2 from \cite{Kominek89}, that $g$ is close to an additive function $h\colon\R^n\to\R$ on all points inside the small ball. 
We argue that in the YES case, if $f$ is close to some additive function then for every $\bm p\in \ball(\bm 0,n)$\vnote{$\sqrt{n}$ suffices here, right?} (where most of the probability mass is) we have $|f(\bm p)-h(\bm p)|\leq n^2\delta$. 
While in the NO case since $f$ is far from any additive function, it is also far from $h$. and therefore 
\[\Pr_{\bm p\sim\cN(\bm 0,I)}[|f(\bm p)-h(\bm p)|>2n^2\delta]\geq \varepsilon.\]
And also 
\[\Pr_{\bm p\sim\cN(\bm 0,I)}[|f(\bm p)-h(\bm p)|>2n^2\delta\mid \bm p\in\ball(\bm 0,n)]\geq \frac{3}{4}\varepsilon.\]

%elsewhere because $g$ is defined by extrapolating the value of $g$ within this ball. Therefore, 
We will focus on proving the $100\delta$-additivity of $g$ within $\ball(\bm 0,R)$.
\begin{lem}\label{lem:g-additive-in-ball}
  Suppose that ~\autoref{lem:f-additive-whp} holds. For every $\bm p,\bm q \in \mathbb{R}^n$ with $\|\bm p\|_2, \|\bm q\|_2, \|\bm p + \bm q\|_2 \leq R$, it holds that \[\left|g(\bm p + \bm q) -g(\bm p) - g(\bm q)\right|\leq 30\delta.\]
\end{lem}

The proof of this lemma will crucially rely on the following two lemmas, which say that the conclusions of \autoref{lem:f-additive-whp} hold with high probability, even when one of the points are fixed to a point $\bm p \in \ball(\bm 0,R)$. A consequence of this is that we will be able to query $g$ within a small error, with high probability.




\begin{thm}{(W.h.p. Median is close to majority, if most of the values are close)}\label{thm:median-is-close}
For any $\bm p\in\mathbb{R}^n$, with $g(\bm{p})=\mathsf{median}_{\bm{q}\sim\mathcal{N}(\bm{0},I)}\{g_{\bm{q}}(\bm{p})\}$, if we have for every $\eta\in\left[0,\frac{1}{4}\right]$, and for any $\delta\in\mathbb{R}$, $$\Pr_{\bm{q}_1,\bm{q}_2\sim\mathcal{N}(\bm{0},I)}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|<\delta]>1-\eta,$$ then we claim $$\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|<\delta]>1-4\eta.$$
\end{thm}
\begin{proof}
Define $S_{\leq}\triangleq\{\bm q\in\mathbb{R}^n:g_{\bm q}(\bm p)\leq g(\bm p)\}$, and $S_{\geq}\triangleq\{\bm q\in\mathbb{R}^n:g_{\bm q}(\bm p)\geq g(\bm p)\}$. Since, $g(\bm{p})$ is the median of the set $\{g_{\bm{q}}(\bm{p}):\bm{q}\in\mathbb{R}^n\}$ over $\bm q\sim\cN(\bm 0,I)$, we claim,
\begin{equation}\label{eq:equiprob}
    \Pr_{\bm q\sim\cN(\bm 0,I)}\left[\bm q\in S_{\leq}\right]=\Pr_{\bm q\sim\cN(\bm 0,I)}\left[\bm q\in S_{\geq}\right]=\frac{1}{2}.
\end{equation}
Let it be the case that
\begin{equation}\label{eq:premise}
\begin{split}
    & \Pr_{\bm{q}_1,\bm{q}_2\sim\mathcal{N}(\bm{0},I)}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|<\delta]  >1-\eta,\\
    \equiv &\Pr_{\bm{q}_1,\bm{q}_2\sim\mathcal{N}(\bm{0},I)}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|\geq\delta] \leq\eta,
\end{split}
\end{equation}
but
\begin{equation}\label{eq:conclusion}
\begin{split}
    &\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|<\delta]\leq 1-4\eta.\\
    \equiv &\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta]>4\eta.
\end{split}
\end{equation}

From \eqref{eq:conclusion},  we can say if we randomly sample a vector $\bm q_1\sim\cN(\bm 0,I)$, with probability more than $2\eta$, $g_{\bm{q}_1}(\bm p)$ will be at least $\delta$-far from $g(\bm p)$. Depending on whether, $\bm q_1\in S_{\leq}$, or $\bm q_1\in S_{\geq}$, we show that if we randomly sample another vector $\bm q_2\sim\cN(\bm 0,I),g_{\bm q_2}(\bm p)$ will be at least $\delta$-far from $g_{\bm q_1}(\bm p)$, with probability more than $\eta$. This would be a contradiction to \eqref{eq:premise}, thus proving our claim.

Let $\bm q_1\in S_{\leq}$, i.e. $g_{\bm q_1}(\bm p)\leq g(\bm p)$, and $|g(\bm p)-g_{\bm q_1}(\bm p)|\geq \delta$. Now for all $\bm q_2\in S_{\geq}$, we have 

\[ |g_{\bm q_2}(\bm p)-g_{\bm q_1}(\bm p)|\geq |g_{\bm q_2}(\bm p)-g(\bm p)| +  |g(\bm p)-g_{\bm q_1}(\bm p)|\geq 0 + \delta = \delta.\]

Similarly, if $\bm q_1\in S_{\geq}$, i.e. $g_{\bm q_1}(\bm p)\geq g(\bm p)$, and $|g_{\bm q_1}(\bm p)-g(\bm p)|\geq \delta$, we have for all $\bm q_2\in S_{\leq}$, 

\[ |g_{\bm q_2}(\bm p)-g_{\bm q_1}(\bm p)|\geq |g_{\bm q_2}(\bm p)-g(\bm p)| +  |g(\bm p)-g_{\bm q_1}(\bm p)|\geq 0 + \delta = \delta.\]
So, we may claim
\begin{align*}
    &\Pr_{\bm q_1,\bm q_2\sim\cN(\bm 0,I)}[|g_{\bm q_1}(\bm p)-g_{\bm q_2}(\bm p)|\geq\delta]\\
    &\geq\Pr_{\bm q_1\sim\cN(\bm 0,I)}[\bm q_1\in S_{\leq}]\cdot\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta\mid\bm q_1\in S_{\leq}]\cdot\Pr_{\bm q_2\sim\cN(\bm 0,I)}[\bm q_2\in S_{\geq}]\\
    &+\Pr_{\bm q_1\sim\cN(\bm 0,I)}[\bm q_1\in S_{\geq}]\cdot\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta\mid\bm q_1\in S_{\geq}]\cdot\Pr_{\bm q_2\sim\cN(\bm 0,I)}[\bm q_2\in S_{\leq}]\\
    &=\frac{1}{4}\left(\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta\mid\bm q_1\in S_{\leq}] + \Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta\mid\bm q_1\in S_{\geq}]\right) . \tag{By \eqref{eq:equiprob}}\\
    &=\frac{1}{4}\left(\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta]\right)\\
    &>\frac{4\eta}{4}=\eta. \tag{By \eqref{eq:conclusion}}
\end{align*}
This completes the proof.
%This allows us to claim at least half of the elements in $S$ are at least $\delta$-far from a randomly sampled element from $S$, with probability more than $2\eta$. Let us denote the randomly sampled element by $g_{\bm{q}_1}(\bm{p}),\bm{q}_1\sim\mathcal{N}(\bm{0},I)$. Let us denote by $S'$, the set of $\bm q_2\in\mathbb{R}^{n}:g_{\bm q_2}(\bm p)$ is at least $\delta$-far from $g_{\bm{q}_1}(\bm{p})$, with probability more than $2\eta$. Then, we get for every $\bm{q}_1\sim\mathcal{N}(\bm{0},I)$,
%$$\Pr_{\bm q_1,\bm{q}_2\sim\mathcal{N}(\bm{0},I)}[|g_{\bm{q}_2}(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta]\geq\underbrace{\Pr_{\bm{q_2\sim\mathcal{N}(\bm{0},I)}}\left[\bm{q_2}\in S'\right]}_{\geq\frac{1}{2}}\cdot\underbrace{\Pr_{\bm{q}_2\sim\mathcal{N}(\bm{0},I)}\left[|g_{\bm{q}_2}(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta\mid\bm{q}_2\in S'\right]}_{> 2\eta}>\eta.$$
%$$\implies\Pr_{\bm{q}_1,\bm{q}_2\sim\mathcal{N}(\bm{0},I)}[|g_{\bm{q}_2}(\bm{p})-g_{\bm{q}_1}(\bm{p})|\geq\delta]>\eta,$$ which is a contradiction to our premise. Hence, the claim holds.
\end{proof}

We get an immediate, and useful corollary from \autoref{thm:median-is-close}:

\begin{cor}{(Median is close to majority over scaled gaussians as well, if values over scaled gaussians are close enough )}\label{cor:Median-of-scaled-gaussian-is-also-close}
For any $\bm p\in\mathbb{R}^n$, with $g(\bm{p})=\mathsf{median}_{\bm{q}\sim\mathcal{N}(\bm{0},I)}\{g_{\bm{q}}(\bm{p})\}$, if we have for every $\eta\in[0,\frac{1}{2}]$, and for any $\delta\in\mathbb{R}$,
$$\Pr_{\bm{q}_1,\bm q_2\sim\mathcal{N}(\bm{0},I)}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|<\delta]>1-\eta,$$ and
$$\Pr_{\substack{\bm{q}_1\sim\mathcal{N}(\bm{0},(1/2)I)\\ \bm q_2\sim\cN(\bm 0,I)}}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|<\delta]>1-\eta,$$
then we claim
$$\Pr_{\bm{q}_1\sim\mathcal{N}(\bm{0},(1/2)I)}[|g(\bm{p})-g_{\bm{q}_1}(\bm{p})|<2\delta]>1-5\eta.$$
\end{cor}
\begin{proof}
Let us define the set $S\triangleq\{\bm q\in\mathbb{R}^n:|g(\bm p)-g_{\bm q}(\bm p)|\geq\delta\}$. Since we have
\begin{equation*}
\begin{split}
    &\Pr_{\bm{q}_1,\bm q_2\sim\mathcal{N}(\bm{0},I)}[|g_{\bm{q}_1}(\bm{p})-g_{\bm{q}_2}(\bm{p})|<\delta]>1-\eta,\\
    \equiv &\Pr_{\bm q_1,\bm q_2\sim\cN(\bm 0,I)}[|g_{\bm q_1}(\bm p)-g_{\bm q_2}(\bm p)|\geq\delta]\leq\eta,
\end{split}
\end{equation*}
by \autoref{thm:median-is-close}, we claim
\begin{equation}
\begin{split}
    \Pr_{\bm q\sim\cN(\bm 0,I)}[\bm q\in S]\leq 4\eta.
\end{split}
\end{equation}
If we randomly sample vectors $\bm {q_1}\sim\cN(\bm 0,(1/2)I),\bm {q_2}\sim\cN (\bm 0,I)$, 
by our premise, $g_{\bm q_1}(\bm p)$ is at least $\delta$-far from $g_{\bm q_2}(\bm p)$, with probability at most $\eta$, and $g_{\bm q_2}(\bm p)\in S$,
i.e. $g_{\bm q_2}(\bm p)$ itself is at least $\delta$-far from $g(\bm p)$, with probability at most $4\eta$. By a union bound, we have
\begin{equation*}
\begin{split}
    \Pr_{\bm q_1\sim\cN(\bm 0,(1/2)I)}[|g(\bm p)-g_{\bm q_1}(\bm p)|\geq 2\delta]& \leq\Pr_{\substack{\bm q_1\sim\cN(\bm 0,(1/2)I)\\ \bm q_2\sim\cN(\bm 0,I)}}[|g_{\bm q_1}(\bm p)-g_{\bm q_2}(\bm p)|\geq\delta] + \Pr_{\bm q_2\sim\cN(\bm 0,I)}[\bm q_2\in S]\\
    &\leq \eta + 4\eta = 5\eta.\\
    \implies\Pr_{\bm q_1\sim\cN(\bm 0,(1/2)I)}[|g(\bm p)-g_{\bm q_1}(\bm p)|< 2\delta]& >1-5\eta.
\end{split}
\end{equation*}
This complete the proof.
\end{proof}

\begin{lem}\label{lem:g-is-well-defined}
  Suppose that \autoref{lem:f-additive-whp} holds, then  for every $\bm p \in \mathbb{R}^n$ with $\|\bm p\|_2 \leq R$,
  \begin{equation}\label{eq:g_is_approximated_majority_gaussian}
      \Pr_{\bm x \sim \mathcal{N}(\bm 0,I)}[|g(\bm p) - ( f(\bm p-\bm x) + f(\bm x))|<6\delta] \geq \frac{76}{100}.
  \end{equation}
  
  Furthermore, 
   \begin{equation}\label{eq:g_is_approximated_majority_scaled_gaussian}
      \Pr_{\bm x \sim \mathcal{N}(\bm 0,(1/2)I)}[|g(\bm p) - ( f(\bm p-\bm x) +f(\bm x))|<12\delta] \geq \frac{7}{10}.
  \end{equation}

\end{lem}
\begin{proof}
  Fix a point $\bm p \in \mathbb{R}^n$ with $\|\bm p\|_2 \leq R$. We will bound the following probability which can be thought as approximate-collision probability for  $i=1$ and for $i=1/2$.
  \[ A:= \Pr_{\bm x \sim \mathcal{N}(\bm 0,I),\bm y\sim \mathcal{N}(\bm 0,iI)} [|(f(\bm p-\bm x) + f(\bm x))-( f(\bm p -\bm y) +f(\bm y))|\leq 6\delta].\]
  Observe that
  \begin{align*}
    1-A=& \Pr_{\bm x \sim \mathcal{N}(0,I),\bm y\sim \mathcal{N}(0,iI)}[|f(\bm x) - f(\bm y) -f(\bm p - \bm y) + f(\bm p-\bm x)|\geq 6\delta ]\\
    \leq & \Pr_{\bm x \sim \mathcal{N}(0,I),\bm y\sim \mathcal{N}(0,iI)}[|f(\bm x) - f(\bm y) - f(\bm x-\bm y)|>\delta ] \\
    &+ \Pr_{\bm x \sim \mathcal{N}(0,I),\bm y\sim \mathcal{N}(0,iI)}[|f(\bm x-\bm y) - f(\bm p-\bm y) + f(\bm p-\bm x)|>5\delta] \\
    < & \frac{1}{100} + \Pr_{\bm x \sim \mathcal{N}(0,I),\bm y\sim \mathcal{N}(0,iI)}[|f(\bm x-\bm y) - f(\bm p-\bm y) + f(\bm p-\bm x)|>5\delta] \tag{By \autoref{lem:f-additive-whp} \eqref{eq:lem3-3} and \eqref{eq:lem3-4}}
  \end{align*}
  It remains to bound the second term. Intuitively, because $\bm x-\bm p\sim\cN(-\bm p, I), \bm y-\bm p \sim \mathcal{N}(-\bm p, iI)$ and  $\bm p \approx 0$, the random variables $\bm x-\bm p$ and $\bm y-\bm p$ should be distributed similarly to $\bm x$ and $\bm y$. Indeed,
  \begin{align*}
    &\Pr_{\bm x \sim \mathcal{N}(0,I),\bm y\sim \mathcal{N}(0,iI)}[|f(\bm x-\bm y) -( f(\bm p-\bm y) - f(\bm p-\bm x))|>5\delta] \\
    =& \Pr_{\bm x \sim \mathcal{N}(0,I),\bm y\sim \mathcal{N}(0,iI)}[|f(\underbrace{\bm x-\bm p}_{\triangleq \bm{r_1}} -(\underbrace{\bm y-\bm p}_{\triangleq \bm{r_2}})) -( f(\bm p-\bm y) - f(\bm p-\bm x))|>5\delta] \\
    =&\Pr_{\bm {r_1} \sim \mathcal{N}(-\bm p,I),\bm {r_2}\sim \mathcal{N}(-\bm p,iI)}[|f(\bm{r_1}-\bm{r_2}) - (f(-\bm{r_2}) - f(-\bm{r_1}))|>5\delta] \\
    \leq & \Pr_{\bm {r_1} \sim \mathcal{N}(0,I),\bm {r_2}\sim \mathcal{N}(0,iI)}[|f(\bm{r_1}-\bm{r_2}) -( f(-\bm{r_2}) - f(-\bm{r_1}))|>5\delta]\\
    &+ 2\Big(\underbrace{\dtv \Big(\mathcal{N}(\bm 0, I), \mathcal{N}(-\bm p, I) \Big)}_{\leq 1/100,\; by \; \autoref{lem:usefulDTVBound}} + \underbrace{\dtv \Big(\mathcal{N}(\bm 0, iI), \mathcal{N}(-\bm p, iI) \Big)}_{\leq i/100,\; by \; \autoref{lem:usefulDTVBound}}\Big) \\
     \leq & \Pr_{\bm {r_1} \sim \mathcal{N}(0,I),\bm {r_2}\sim \mathcal{N}(\bm 0,iI)}[|f(\bm{r_1}-\bm{r_2}) - f(\bm{r_1}) + f(\bm{r_2})|>\delta] + \frac{1}{100}+ \frac{i}{100} \\
    &+  \Pr_{\bm{r_1} \sim \mathcal{N}(\bm 0, I)}[ |f(-\bm{r_1}) - f(\bm{r_1})|>2\delta]+\Pr_{\bm{r_2} \sim \mathcal{N}(\bm 0, iI)}[ |f(-\bm{r_2}) - f(\bm{r_2})|>2\delta] \tag{Claim~\ref{clm:tvd-bound-on-ball}} \\
    \leq & \frac{3}{100} +  \frac{1}{100} +\frac{i}{100} \leq \frac{5}{100}. \tag{By  ~\eqref{eq:lem3-1}-~\eqref{eq:lem3-4} in Lemma~\ref{lem:f-additive-whp}}
  \end{align*}
  Plugging this into our previous bound on $A$, we can conclude that
 
   \[ A \geq 1- \left(\frac{1}{100} + \frac{5}{100} \right) = 1 - \frac{6}{100}.  \]
   
   \[ \equiv \Pr_{\substack{\bm x \sim \cN (\bm 0, I) \\ \bm y \sim \cN (\bm 0,iI)}}[|g_{\bm x}(\bm p) - g_{\bm y}(\bm p)| > 6\delta] <\frac{6}{100} \]

 
  Applying \autoref{thm:median-is-close} we conclude that for every $\bm p\in\ball(\bm 0,R)$ 
  %\vnote{For $i=1$, it works, but not for $i=1/2$, since $g(\bm p)$ is the median of $S=\{g_{\bm q}(\bm p) : \bm q \sim \cN (\bm 0, I)\}$, but we are trying to show it will be close to the majority of values in $S'=\{g_{\bm q}(\bm p) : \bm q \sim \cN (\bm 0, I/2)\}$. And, we know $\dtv(\cN (\bm 0,I),\cN (\bm 0,I/2))$ is large.}
  \[\Pr_{\bm q \sim \mathcal{N}(\bm 0, I)} [|g(\bm p) - (f(\bm p -\bm q) +f(\bm q))|\leq 6\delta] \geq 76/100.\]
  For $i=1/2$, applying \autoref{cor:Median-of-scaled-gaussian-is-also-close}, we conclude that for every $\bm p\in\ball(\bm 0,R)$,
\[\Pr_{\bm q \sim \mathcal{N}(\bm 0,(1/2) I)} [|g(\bm p) - (f(\bm p -\bm q) +f(\bm q))|\leq 12\delta] \geq 7/10.\]
\end{proof}






The following lemma is essentially condition~\eqref{eq:lem3-3} of Lemma~\ref{lem:f-additive-whp} with two fixed points.

\begin{lem}\label{lem:whp-g-additive-two-points}
  Suppose that ~\autoref{lem:f-additive-whp} holds then, for every $\bm p,\bm q \in \mathbb{R}^n$ with $\|\bm p\|_2, \|\bm q\|_2, \|\bm p+\bm q\| \leq R$,
  \[ \Pr_{\bm{x,y,z} \sim \mathcal{N}(\bm 0, I)} \Big[ \left|g(\bm p + \bm q) -\left( f \Big(\bm p - \frac{\bm x-\bm z}{2} \Big) + f \Big( \bm q - \frac{\bm z-\bm y}{2} \Big) + f \Big( \frac{\bm x-\bm y}{2} \Big)\right)\right|>15\delta \Big] \leq  \frac{4}{10}. \]
\end{lem}

\begin{proof}
  Fix a pair of points $\bm p,\bm q \in \mathbb{R}^n$ with $\|\bm p\|_2, \|\bm q\|_2 \leq R$. We can bound the probability
  \begin{align*}
    &\Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(\bm 0, I)} \Big[\left| g(\bm p + \bm q) -\left( f \Big(\bm p - \frac{\bm x-\bm z}{2} \Big) + f \Big( \bm q - \frac{\bm z-\bm y}{2} \Big) + f \Big( \frac{\bm x-\bm y}{2} \Big) \right)\right|>15\delta\Big] \\
    \leq &\Pr_{\bm x,\bm y \sim \mathcal{N}(\bm 0, I)} \Big[ \left|g(\bm p+\bm q) -\left( f \Big(\bm  p+\bm q - \frac{\bm x-\bm y}{2} \Big) + f \Big( \frac{\bm x-\bm y}{2} \Big) \right)\right|>12\delta\Big] \\
    &+ \Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(\bm 0, I)} \Big[ \left|f \Big(\bm  p +\bm  q - \frac{\bm x-\bm y}{2} \Big) -\left( f \Big(\bm  p - \frac{\bm x-\bm z}{2} \Big) + f \Big(\bm  q -\frac{\bm z-\bm y}{2} \Big)\right)\right|>3\delta \Big]
  \end{align*}
  To bound the first term, observe that if $\bm x,\bm y \sim \mathcal{N}(\bm 0, I\bm )$, then the random variable $(\bm x-\bm y)/2$ is  distributed according to $\mathcal{N}(\bm 0,(1/2) I)$. Furthermore, because $\|\bm p+\bm q \|_2 \leq R$,  we can apply ~\autoref{lem:g-is-well-defined} \eqref{eq:g_is_approximated_majority_scaled_gaussian} and conclude that
  \begin{align*}
    &\Pr_{\bm x,\bm y \sim \mathcal{N}(\bm 0, I)} \Big[ \left|g(\bm p +\bm  q) -\left( f \Big(\bm p +\bm  q -  \frac{\bm x-\bm y}{2} \Big) + f \Big(\frac{\bm x-\bm y}{2} \Big)\right)\right|>12\delta \Big] \\
    =& \Pr_{\bm r\sim \mathcal{N}(\bm 0,(1/2) I)} \Big[ \left|g(\bm p +\bm  q) -\left( f ((\bm p +\bm  q) -  \bm r ) + f (\bm r )\right)\right|>12\delta \Big]\leq \frac{3}{10}.
  \end{align*}
  To bound the second term, observe that
  \begin{align*}
    &\Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(\bm 0, I)} \Big[\left| f \Big(\bm  p +\bm  q - \frac{\bm x-\bm y}{2} \Big) -\left( f\Big(\bm p- \frac{\bm x-\bm z}{2} \Big) + f\Big(\bm q- \frac{\bm z-\bm y}{2} \Big)\right)\right|>3\delta \Big] \\
    =&\Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(\bm 0, I)} \left[ \left|f \left(\frac{(2\bm q +\bm y)-(\bm x-2\bm p)}{2} \right) -\left(f \left( \frac{(2\bm q +\bm y)-\bm z}{2} \right) + f \left( \frac{\bm z-(\bm x-2\bm p)}{2} \right)\right)\right|>3\delta \right] \\
    =&\Pr_{\substack{\bm x \sim \mathcal{N}(-2\bm p,I) \\\bm  y \sim \mathcal{N}(2\bm q,I) \\ \bm z \sim \mathcal{N}(\bm 0,I)}}\Big[ \left|f \Big(\frac{\bm y-\bm x}{2} \Big) -\left( f \Big( \frac{\bm y-\bm z}{2} \Big) + f\Big( \frac{\bm z-\bm x}{2} \Big)\right)\right|>3\delta \Big] \\
    \leq  &\Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(\bm 0, I)}\Big[\left| f \Big(\frac{\bm x-\bm y}{2} \Big) -\left( f \Big( \frac{\bm x-\bm z}{2} \Big) + f \Big( \frac{\bm z-\bm y}{2} \Big)\right)\right| \Big]  + \dtv \Big( \mathcal{N}(\bm 0, I), \mathcal{N}(-2\bm p, I )\Big) \\&+  \dtv \Big( \mathcal{N}(\bm 0,I), \mathcal{N}(2\bm q, I )\Big) \\
    \leq & \frac{1}{100} + \frac{2}{100} + \frac{2}{100} = \frac{5}{100}. \tag{By Lemma~\ref{lem:f-additive-whp} \eqref{eq:lem3-3} and Claim~\ref{clm:tvd-bound-on-ball}}
  \end{align*}
  Combining both of these bounds, we have
  \[\Pr_{\bm x,\bm y,\bm z \sim \mathcal{N}(\bm 0,I)} \left[ \left|g\left(\bm p +\bm  q\right) -\left( f \left(\bm p - \frac{\bm x-\bm z}{2} \right) + f \left(\bm  q - \frac{\bm z-\bm y}{2} \right) + f \left(\frac{\bm x-\bm y}{2} \right)\right)\right|>15\delta \right]
  \leq 3/10+5/100 \leq 4/10.\]
\end{proof}


The additivity of $g$ within $\ball(\bm 0,R)$ is an immediate consequence of these two lemmas.

\begin{proof}[Proof of Lemma~\ref{lem:g-additive-in-ball}]
  Let $\bm p,\bm q \in \mathbb{R}^n$ be any pair of points satisfying $\|\bm p\|_2, \|\bm q\|_2, \|\bm p + \bm q\|_2 \leq R$. Our aim is to show that $\left|g(\bm p + \bm q) - g(\bm p) - g(\bm q)\right|\leq 30\delta$. By a union bound we show that the probability that $\bm x,\bm y,\bm z \sim \mathcal{N}(0,I)$ simultaneously satisfy
  \begin{enumerate}
    \item $\left|g(\bm p + \bm q) -\left( f(\bm p - \frac{\bm x - \bm z}{2}) + f(\bm  q - \frac{\bm z - \bm y}{2} ) + f(\frac{\bm x - \bm y}{2})\right)\right|<15\delta$,\label{itm:itm-1}
    \item $\left|g(\bm p) -\left( f(\bm p - \frac{\bm x - \bm z}{2} ) + f(\frac{\bm x - \bm z}{2})\right)\right|<6\delta$\label{itm:itm-2},
    \item $\left| g(\bm q) -\left( f(\bm q - \frac{\bm z - \bm y}{2}) + f( \frac{\bm z - \bm y}{2})\right)\right|<6\delta$,\label{itm:itm-3}
    \item $\left|f(\frac{\bm x - \bm y}{2}) -\left(f(\frac{\bm x - \bm z}{2}) - f (\frac{\bm z - \bm y}{2})\right)\right|<3\delta$\label{itm:itm-4}
  \end{enumerate}
  is at least $1- (4/10+ 2\cdot 2/10  + 1/100)  > 0$. \autoref{itm:itm-1} is by \autoref{lem:whp-g-additive-two-points} and \autoref{itm:itm-4} is by \autoref{lem:f-additive-whp} \eqref{eq:lem3-3} . For \autoref{itm:itm-2} and \autoref{itm:itm-3} we are using the fact that $((\bm x - \bm y)/2),((\bm x - \bm z)/2)\text{, and }((\bm z - \bm y)/2)$ are distributed as $\mathcal{N}(0,(1/2)I)$ and apply \autoref{lem:g-is-well-defined}\eqref{eq:g_is_approximated_majority_scaled_gaussian}.
  Fixing such a triple $(\bm x,\bm y,\bm z)$, we conclude that
  \begin{align*}
    |g(\bm p + \bm q)-g(\bm p)-g(\bm q)|\leq & 
    \left|g ( \bm p + \bm q) - f \Big(\bm p - \frac{\bm x - \bm z}{2} \Big) - f \Big( \bm q - \frac{\bm z - \bm y}{2} \Big) - f \Big (\frac{\bm x - \bm y}{2} \Big)\right| \\
    &+\left| f \Big(\bm p - \frac{\bm x - \bm z}{2} \Big) +f \Big( \bm q - \frac{\bm z - \bm y}{2} \Big) +f \Big (\frac{\bm x - \bm y}{2} \Big)-g(\bm p) - g(\bm q) \right| \\
    \leq& 15\delta+\left| f \Big(\bm p - \frac{\bm x - \bm z}{2} \Big)+ f \Big(\frac{\bm x - \bm z}{2}\Big) -g(\bm p)\right|\\ &+\left|f \Big( \bm q - \frac{\bm z - \bm y}{2} \Big)+  f \Big( \frac{\bm z - \bm y}{2} \Big)- g(\bm q)\right|+\left|f \Big (\frac{\bm x - \bm y}{2} \Big)- f \Big(\frac{\bm x - \bm z}{2} \Big) -  f \Big( \frac{\bm z - \bm y}{2} \Big)\right|\\
    \leq& 30\delta.
  \end{align*}
  Therefore $g$ is additive within $\ball(\bm 0,R)$.
\end{proof}

Finally, we argue that $g$ is close to an additive function $h$ inside the large ball. 
%Intuitively this should be true because the values of $g$ on points outside of $\ball (0,1/r)$ are defined by extrapolating the values of $g$ on points within $\ball (0,1/r)$, where we know $g$ is additive. For the proof, it will be useful to record the following fact.
%   \begin{fact}\label{fact:g-homogeneous-over-ball}
%   	 Provided that~\eqref{eq:lem3-1} --~\eqref{eq:lem3-3} of Lemma~\ref{lem:f-additive-whp} hold then, for  every $\bm p \in \mathbb{R}^n$ with $\| \bm p \|_2 \leq R$ and $c \in \mathbb{Z}_{> 0}$, we have  $g(\bm p) = c g(\bm p/c)$.
%   \end{fact}
%   \begin{proof} Observe that
%   $g(\bm p) = g((c/c)\bm p) = g \left( \sum_{i=1}^c \bm p/c \right) = \sum_{i=1}^c g(\bm p/c) =  c \cdot g(\bm p/c)$, where the third equality follows by Lemma~\ref{lem:g-additive-in-ball}, noting that $\|kp/c\|_2 \leq 1/r$ for every $k \in [c-1]$
%   \end{proof}

\begin{proof}
  [Proof of Lemma~\ref{lem:g-is-additive}]
  $g$ is $30\delta$-additive by \autoref{lem:g-additive-in-ball}. 
  $g_{\bm x}(\bm p)$ is a good estimation (up to $6\delta$) for $g(\bm p)$ with high probability $\left(\frac{76}{100}>\frac{1}{2}\right)$ for $x\sim\cN(\bm 0,I)$ by \autoref{lem:g-is-well-defined}.
%   Fix a pair of points $p,q \in \mathbb{R}^n$, we will argue that $g(p+q) = g(p) + g(q)$. Recall that $g(p):= k_p g(p/k_p)$, $g(q):= k_q g(q/k_q)$, and $g(p+q):= k_{p+q} g((p+q)/k_{p+q})$. Then,
%   \[ g(p)+g(q) = k_p \cdot g\left( \frac{p}{k_p} \right) + k_q \cdot g\left( \frac{p}{k_q} \right) = k_p k_q k_{p+q} \cdot g\left( \frac{p}{k_p k_q k_{p+q}} \right) + k_p k_q k_{p+q} \cdot g\left( \frac{p}{k_p k_q k_{p+q}} \right),  \]
%   where the second equality follows by Fact~\ref{fact:g-homogeneous-over-ball}, noting that $k_p, k_q, k_{p+q} \in \mathbb{Z}^{> 0}$ and so $p/k_p, q/k_q \in \ball(0,1/r)$. Furthermore, because $p/(k_p k_q k_{p+q}), q/(k_p k_q k_{p+q}),(p+q)/ (k_p k_q k_{p+q}) \in \ball(0,1/r)$, we can apply Lemma~\ref{lem:g-additive-in-ball} to obtain
%   \begin{align*} k_p k_q k_{p+q} \left( g\left( \frac{p}{k_p k_q k_{p+q}} \right) + g\left( \frac{p}{k_p k_q k_{p+q}} \right) \right) &= k_p k_q k_{p+q} \cdot g\left( \frac{p+q}{k_p k_q k_{p+q}} \right) \\
%   &= k_{p+q} \cdot g\left( \frac{p+q}{k_{p+q}} \right) \\
%   &=g(p+q),
%   \end{align*}
%   where the second equality follows by Fact~\ref{fact:g-homogeneous-over-ball}, noting that $k_p k_q \in \mathbb{Z}^{>0}$ and $(p+q)/k_{p+q} \in \ball(0,1/r)$.

%   Finally, by Lemma~\ref{lem:g-is-well-defined}, $g$ is well-defined within $\ball(0,1/r)$. Because $g$ is defined by extrapolating from its value within this ball, it is well-defined everywhere.
  %Then,
  %\[ g(p)+g(q) = k_p \cdot g\left( p/k_p \right) + k_q \cdot g\left( \frac{p}{k_q} \right) = k_p k_q \cdot g\left( \frac{p}{k_p k_q} \right) + k_p k_q \cdot g\left( \frac{p}{k_p k_q} \right),  \]
  %where the second equality follows by Lemma~\ref{lem:g-additive-in-ball}, noting that $k_p, k_q \in \mathbb{Z}^{\neq 0}$ and so $\| p/ (k_p k_q) \|_2 \leq \|p/k_p \|_2$ and $\| q/ (k_p k_q) \|_2 \leq \|q/k_p \|_2$ and so $k_p k_q p, k_p k_q p \in \ball(0,1/r)$.
  %To conclude, we consider several cases based on whether $p$, $q$ and $p+q$ are in $\ball(0,1/r)$ or not.
  %\begin{enumerate}
  % \item If $p,q \in \ball(0,1/r)$, then $k_p, k_q = 1$. Let $g(p+q) := k_{p+q} g((p+q)/k_{p+q})$, because $1/k_{p+q}\leq 1$, $\| p/ k_{p+q} \|_2 \leq \| p\|_2$ and $\|q/k_{p+q} \|_2 \leq \|q\|_2$. Therefore, because $k_{p+q} \in \mathbb{Z}^{\neq0}$ and $(p+q)/k_{p+q} \in \ball(0,1/r)$, by Lemma~\ref{lem:g-additive-in-ball},
  %   \[ k_{p+q} \cdot g \left( \frac{p}{k_{p+q}} \right)+ k_{p+q} \cdot g \left( \frac{q}{k_{p+q}} \right) = k_{p+q} \cdot g \left( \frac{p+q}{k_{p+q}} \right) = g(p+q) \]
  % \item If $p,q \in \ball(0,1/r)$ and $p+q \not \in \ball(0,1/r)$, then $g(p+q) = k_{p+q}$
  % \item If $p \in \ball(0,1/r)$, $q \not \in \ball(0,1/r)$, then by the definition of $k_q$, $q/ k_q \in \ball(0,1/2r)$. It follows that $p/k_q \in \ball(0,1/2r)$ and
  % $p/(k_p k_q), q/ (k_p k_q) \in \ball(0,1/2r)$.
  % Thus, $\|(p+q)/(k_p k_q) \|_2 \leq \|p/k_p k_q\|_2 + \|q/ k_p k_q\|_2 \leq 1/r$
  % and so $(p+q)/(k_pk_q) \in \ball(0,1/r)$ and we can apply Lemma~\ref{lem:g-additive-in-ball}.
  %\end{enumerate}
  %Now, let $\lambda_1, \lambda_2 \in \mathbb{Z}$ be such that $\lambda_1 k_{p+q} = \lambda_2 k_p k_q$. Note that such $\lambda_1, \lambda_2$ exist because because $k_q k_q, k_{p+q} \in \mathbb{Z}^{\neq 0}$.
  %Furthermore, because $(p+q) / k_{p+q}, (p+q)/k_p k_q \in \ball(0,1/r)$, both $(p+q)/(\lambda_1 k_{p+q})$ and $(p+q)/(\lambda_2 k_q)$ are within $\ball(0,1/r)$. Therefore,
  %\begin{enumerate}
  % \item $p,q, p+q \in \ball(0,1/r)$: By Lemma~\ref{lem:g-additive-in-ball} $g(p+q) = g(p) + g(q)$.
  % \item $p,q \in \ball(0,1/r)$, $p+q \not \in \ball(0,1/r)$: In this case, $g(p +  q) := k_{p+q}g \big(\frac{p+q}{k_{p+q}} \big)$. By definition, $\frac{p+q}{k_{p+q}} \in \ball(0,1/r)$. Furthermore, because $1/k_{p+q} < 1$, we have that $\frac{p}{k_{p+q}}, \frac{q}{k_{p+q}} \in \ball(0,1/r)$. Therefore,
  %   \[g(p+q) = k_{p+q}  \cdot g \left( \frac{p}{k_{p+q}}+ \frac{q}{k_{p+q}} \right) = k_{p+q} \cdot g \left( \frac{p}{k_{p+q}} \right) + k_{p+q} \cdot g \left( \frac{q}{k_{p+q}} \right), \]
  %   and because $k_{p+q} \in \mathbb{Z}$ and $p,q \in \ball(0,1/r)$, we have
  %   $k_{p+q} g \left( \frac{p}{k_{p+q}} \right) +  k_{p+q}  g \left( \frac{q}{k_{p+q}} \right) = g(p) + g(q).  $
  % \item $p \in \ball(0,1/r)$, $q, p+q \not in \ball(0,1/r)$: In this case $g(q):= k_q g \big (\frac{q}{k_q} \big)$ and $g(p +  q) := k_{p+q}g \big(\frac{p+q}{k_{p+q}} \big)$. Then,
  %   \[ g(p) + g(q) = g(p) + k_q g \left( \frac{q}{k_q} \right) =  k_q g \left( \frac{p}{k_q} \right) +  k_q g \left( \frac{q}{k_q} \right) = k_q g \left(\frac{p+q}{k_q} \right), \]
  %   where the second equality follows from the fact that $1/k_q <1$ and so $p/k_q \in \ball(0,1/r)$, along with the fact that $g$ is additive within $\ball(0,1/r)$. Now, let $\lambda_1, \lambda_2 \in \mathbb{Z}$ be such that $\lambda_1 k_{p+q} = \lambda_2 \delta_2$. Note that such $\lambda_1, \lambda_2$ exist because because $k_q, k_{p+q} \in \mathbb{Z}$. Furthermore, because $(p+q) / k_{p+q}, (p+q)/k_q \in \ball(0,1/r)$, both $(p+q)/(\lambda_1 k_{p+q})$ and $(p+q)/(\lambda_2 k_q)$ are within $\ball(0,1/r)$. Therefore,
  %   \begin{align*}
  %     k_q g \left( \frac{p+q}{k_q} \right) = k_q \lambda_2 g \left( \frac{p+q}{k_q \lambda_2} \right) = k_{p+q} \lambda_1 g \left( \frac{p+q}{k_{p+q} \lambda_1} \right) = k_{p+q} g \left ( \frac{p+q}{k_{p+q}} \right) = g(p+q).
  %   \end{align*}
  % \item $p,q,p+q \not \in \ball(0,1/r)$: By the definition of $g$,
  %   \[ g(p) + g(q) = k_p g \left( p/k_p\right) + k_q g \left( \frac{q}{k_q}\right) = k_p k_q g \left( \frac{p}{k_p k_q}\right) + k_p k_q g \left( \frac{q}{k_p k_q}\right) = k_p k_q g \left( \frac{p+q}{k_p k_q}\right), \]
  %   where the second equality follows because $k_p, k_q \in \mathbb{Z}$ and so $k_p k_q p, k_p, k_q q \in \ball(0,1/r)$. Let $\lambda_1, \lambda_2$ be such that
  %\end{enumerate}
\end{proof}


